WPDA: Frequency-based Backdoor Attack with Wavelet Packet Decomposition

This work explores an emerging security threat against deep neural networks (DNNs) based image classification, i.e., backdoor attack. In this scenario, the attacker aims to inject a backdoor into the model by manipulating training data, such that the backdoor could be activated by a particular trigger and bootstraps the model to make a target prediction at inference. Currently, most existing data poisoning-based attacks struggle to achieve success at low poisoning ratios, increasing the risk of being defended by defense methods. In this paper, we propose a novel frequency-based backdoor attack via Wavelet Packet Decomposition (WPD), WPD decomposes the original image signal to a spectrogram that contains frequency information with different semantic meanings. We leverage WPD to statistically analyze the frequency distribution of the dataset to infer the key frequency regions the DNNs would focus on, and the trigger information is only injected into the key frequency regions. Our method mainly includes three parts: 1) the selection of the poisoning frequency regions in spectrogram; 2) trigger generation; 3) the generation of the poisoned dataset. Our method is stealthy and precise, evidenced by the 98.12% Attack Success Rate (ASR) on CIFAR-10 with the extremely low poisoning ratio 0.004% (i.e., only 2 poisoned samples among 50,000 training samples) and can bypass most existing defense methods. Besides, we also provide visualization analyses to explain why our method works.

==> tables/algorithm1.tex <==
\begin{algorithm}[H]
\caption{Selection of Key Regions to Mask}\label{The_algorithm_of_WPDA}
\begin{algorithmic}[1]
\REQUIRE The benign training dataset as $\mathcal{D} = \{\mathbf{x}^{(1)}, \dots, \mathbf{x}^{(n)}\}$, the level of WPD $N$.
\ENSURE The list of key frequency regions $k_{list}$ that will be masked in the training samples.
\end{algorithmic}
\vspace{-0.5em}
\begin{spacing}{1.18}
\begin{multicols}{2}
\begin{algorithmic}[1]
\setlength{\baselineskip}{0.68\baselineskip}
\STATE $k_{list} = []$
\FOR{$p = 1, \dots, 4^{N-1}$} 
    \STATE $s_{list} = []$
    \FOR{$s \leftarrow 1$ \TO 4}
        \STATE \small${C^N_{s,p}} = \left\{\sum\limits_{x^{(i)} \in \mathcal{D}} \mathcal{W}^{N}(x^{(i)}) \right\}_{s,p}$
        \STATE \normalsize $E^N_{s,p} = \left| \text{avg}(C^N_{s,p}) \right|$
        \STATE $s_{list}.append(E^N_{s,p})$
    \ENDFOR
    \IF{$p = 1$}
        \STATE $s_{list}.remove(\max(s_{list}))$ 
        \STATE $p, s^* = \mathop{\arg\max}\limits_{p,s} \{s_{list}\}$
    \ELSE
        \STATE $p, s^* = \mathop{\arg\max}\limits_{p,s} \{s_{list}\}$
    \ENDIF
    \STATE $k_{list}.append(\{p, s^*\})$
\ENDFOR
\RETURN $k_{list}$
\end{algorithmic}
\end{multicols}
\end{spacing}
\vspace{-0.5em}
\label{alg1}
\end{algorithm}


==> tables/algorithm2.tex <==
 
\begin{algorithm*}[H]
\caption{Selection of Critical Frequency Regions to Mask}\label{The algorithm of WPDA}
\begin{algorithmic}[1]
\setlength{\baselineskip}{0.95 \baselineskip}
\REQUIRE The benign training dataset as $\D = \{\x^{(1)}, \dots, \x^{(n)}\}$, the shape of each sample is $M \times M \times 3$, the level of WPD is $N$, and the vanishing moment of the wavelet basis function is $2L$.
% $\mathcal{W}$ denotes the WPD .
\ENSURE The list of critical frequency regions $k_{list}$ that will be masked in the training samples.
 % of s-th sub-spectrogram in p-th parent-spectrogram.

% \FOR{$p\leftarrow 1$ \TO $4^{N-1}$} 
\STATE{$k_{list}=[]$}
\FOR{$\textbf{p} = {1, \dots, 4^{N-1}}$} 
    \STATE{$\textbf{s}_{list}=[]$}
    \FOR{$\textbf{s} = 1$ \TO 4} 
        % \FOR{$s$ in range 4} \do
        \STATE $E^N_{\textbf{p},\textbf{s}} = {\left |{\frac{1}{m \cdot n \cdot 3} \sum\limits_{\x^{(i)}\in \D} \sum_{i=1}^{m} \sum_{j=1}^{n} \sum_{c=1}^{3}} C^N_{\textbf{p},\textbf{s}}(\x^{(i)}) \right |}$
        % {$C^N_{p,s} = \sum\limits_{\x^{(i)}\in \D}^{}{\left[\mathcal{W}^{N}_{p,s}(\x^{(i)})\right]}$}
        % {${C^N_{p,s}} = \{\sum\limits_{x^{(i)}\in \D}^{}{\mathcal{W}^{N}(x^{(i)})\}_{p,s}}$}
        % \STATE{$E^N_{p,s} = {\left |{\frac{1}{m \cdot n \cdot 3} \sum_{i=1}^{m} \sum_{j=1}^{n} \sum_{c=1}^{3}} C^N_{p,s} \right |}$, \\$where \hspace{0.3cm} m = n = \frac{M+2L}{2^N}$}
        % {$E^N_{p,s} = \left |\text{avg}(C^N_{p,s})  \right |$}
        \STATE {$\textbf{s}_{list} \leftarrow \textbf{s}_{list} \cup \{(E^N_{\textbf{p},\textbf{s}},\textbf{p},\textbf{s})\}$}
        \ENDFOR
    \IF{$\textbf{p}=1$}{
        \STATE{$ \textbf{s}_{list} \leftarrow \textbf{s}_{list} \setminus \mathop{\arg\max}\limits_{(E^N_{\textbf{p},\textbf{s}}, \textbf{s}, \textbf{p}) \in \textbf{s}_{\text{list}}} E^N_{\textbf{p},\textbf{s}}$} 
        % {$s_{list} \leftarrow s_{list} \setminus \{\max(s_{{list}})\}$}
        % {$s_{list}={s_{list}}\text{.remove}(\max(s_{list}))$} 
        \STATE{$\textbf{p}, \textbf{s}^*=\mathop{\arg\max}\limits_{(E^N_{\textbf{p},\textbf{s}}, \textbf{s}, \textbf{p}) \in \textbf{s}_{\text{list}}}E^N_{\textbf{p},\textbf{s}}$}}
    \ELSE{
        \STATE{$\textbf{p}, \textbf{s}^*=\mathop{\arg\max}\limits_{(E^N_{\textbf{p},\textbf{s}}, \textbf{s}, \textbf{p}) \in \textbf{s}_{\text{list}}}E^N_{\textbf{p},\textbf{s}}$}}
    \ENDIF
    \STATE {$k_{list} \leftarrow k_{list}\cup \{(\textbf{p}, \textbf{s}^*)\}$}
     

   \ENDFOR
   \RETURN $ k_{list}$
\end{algorithmic}
\label{alg1}
\end{algorithm*}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/complexity_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{Complexity of different datasets in classification tasks. }
\label{complexity_dataset}
\centering
\begin{tabular}{lllll}
\hline
Dataset                   & Model        & $\triangle t$(s) & Accuracy & $C_{dataset}$ \\ \hline \hline
\multirow{2}{*}{CIFAR-10}  &PreAct-ResNet18 & 955     & 0.9408   & 56.536     \\
& VGG19-BN     & 1137    & 0.9238   & 86.6394    \\ \hline
\multirow{2}{*}{CIFAR-100} &PreAct-ResNet18 & 974     & 0.7072   & 285.1872   \\
& VGG19-BN     & 1096    & 0.6589   & 373.8456   \\ \hline
\multirow{2}{*}{Tiny ImageNet}     &PreAct-ResNet18 & 16869   & 0.5733   & 7198.0023  \\
& VGG19-BN     & 12743   & 0.5381   & 5885.9917  \\ \hline
\end{tabular}
\end{table}



==> tables/detection.tex <==
\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{CIFAR-10}. The training model adopts PreAct-ResNet18. }
\label{detection_result_CIFAR-10_pre}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
\\ 
SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.12} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.50} & 0.08 & 0.00 
& \multicolumn{1}{c}{0.20} & 0.08 & 0.00 
& \multicolumn{1}{c}{0.44} & 0.08 & 0.01  
& \multicolumn{1}{c}{0.56} & 0.10 & 0.01  
& \multicolumn{1}{c}{0.94} & 0.12 & 0.13
\\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{CIFAR-10}. The training model adopts VGG19-BN. }
\label{detection_result_CIFAR-10_vgg}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.08 & 0.00
& \multicolumn{1}{c}{0.00} & 0.11 & 0.00
& \multicolumn{1}{c}{0.00} & 0.11 & 0.00
& \multicolumn{1}{c}{0.00} & 0.11 & 0.00
& \multicolumn{1}{c}{0.99} & 0.05 & 0.27
\\ 
SCAn~\cite{tang2021demon}   
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.05 & 0.00
& \multicolumn{1}{c}{0.98} & 0.00 & 0.93  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{1.00} & 0.14 & 0.12
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.00} & 0.10 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.14 & 0.00 
& \multicolumn{1}{c}{0.32} & 0.07 & 0.00  
& \multicolumn{1}{c}{0.42} & 0.09 & 0.01  
& \multicolumn{1}{c}{0.95} & 0.13 & 0.13
\\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{CIFAR-100}. The training model adopts PreAct-ResNet18. }
\label{detection_result_CIFAR-100_pre}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.04 & 0.00
& \multicolumn{1}{c}{0.00} & 0.03 & 0.00
& \multicolumn{1}{c}{0.00} & 0.01 & 0.00
& \multicolumn{1}{c}{0.00} & 0.03 & 0.00
& \multicolumn{1}{c}{0.00} & 0.02 & 0.00
\\ 
SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{1.00} & 0.00 & 1.00  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{1.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{1.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{1.00} & 0.15 & 0.01  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.00} & 0.12 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.13 & 0.00 
& \multicolumn{1}{c}{0.48} & 0.13 & 0.00  
& \multicolumn{1}{c}{0.78} & 0.13 & 0.01  
& \multicolumn{1}{c}{1.00} & 0.13 & 0.14
\\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{CIFAR-100}. The training model adopts VGG19-BN. }
\label{detection_result_CIFAR-100_vgg}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.04 & 0.00
& \multicolumn{1}{c}{0.00} & 0.03 & 0.00
& \multicolumn{1}{c}{0.00} & 0.01 & 0.00
& \multicolumn{1}{c}{0.00} & 0.03 & 0.00
& \multicolumn{1}{c}{0.00} & 0.02 & 0.00
\\ 
SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.05 & 0.00
& \multicolumn{1}{c}{0.98} & 0.00 & 0.93  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.40} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.30} & 0.15 & 0.03
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.00} & 0.13 & 0.14 
& \multicolumn{1}{c}{0.00} & 0.12 & 0.00 
& \multicolumn{1}{c}{0.32} & 0.19 & 0.00  
& \multicolumn{1}{c}{0.42} & 0.17 & 0.01  
& \multicolumn{1}{c}{0.95} & 0.15 & 0.12
\\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{Tiny ImageNet}. The training model adopts PreAct-ResNet18. }
\label{detection_result_tiny_pre}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.01 & 0.00
& \multicolumn{1}{c}{0.00} & 0.01 & 0.00
& \multicolumn{1}{c}{1.00} & 0.01 & 0.12
& \multicolumn{1}{c}{1.00} & 0.01 & 0.26
& \multicolumn{1}{c}{0.00} & 0.02 & 0.00
\\ 
SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.99} & 0.00 & 0.96
& \multicolumn{1}{c}{1.00} & 0.00 & 1.00  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{1.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.40} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.80} & 0.15 & 0.01  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.25} & 0.16 & 0.00 
& \multicolumn{1}{c}{0.40} & 0.13 & 0.00 
& \multicolumn{1}{c}{0.62} & 0.16 & 0.00  
& \multicolumn{1}{c}{0.78} & 0.16 & 0.01  
& \multicolumn{1}{c}{0.96} & 0.18 & 0.10
\\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[!ht]
\caption{The result of WPDA against 4 detection methods under 5 different poisoning ratios in the \textbf{Tiny ImageNet}. The training model adopts VGG19-BN. }
\label{detection_result_tiny_vgg}
\centering
\scriptsize
% \scalebox{1.05}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}{Poisoning ratio $\rightarrow$} & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
  Detection $\downarrow$  & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$   & \multicolumn{1}{c}{TPR}    & FPR    & $F^{\omega}_1$      
\\ 
\hline \hline 
AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.03 & 0.00
& \multicolumn{1}{c}{0.00} & 0.06 & 0.00
& \multicolumn{1}{c}{1.00} & 0.07 & 0.01
& \multicolumn{1}{c}{0.00} & 0.08 & 0.00
& \multicolumn{1}{c}{0.00} & 0.18 & 0.00
\\ 
SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{1.00} & 0.00 & 0.99  
\\ 
Spectral~\cite{tran2018spectral}  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{0.28} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
& \multicolumn{1}{c}{0.17} & 0.15 & 0.01
\\ 
Strip~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.00} & 0.17 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.16 & 0.00 
& \multicolumn{1}{c}{0.10} & 0.13 & 0.00  
& \multicolumn{1}{c}{0.09} & 0.14 & 0.00  
& \multicolumn{1}{c}{0.47} & 0.16 & 0.04
\\
\hline
\end{tabular}
}
\end{table*}

==> tables/detection_Pre.tex <==
% \begin{table}[!ht]
% \caption{The results of WPDA against 3 detection methods on PreAct-ResNet18. }
% \label{detection_result_pre}
% \centering
% % \small
% \large
% % \normalsize
% \renewcommand{\arraystretch}{1.5}
% \scalebox{0.485}{
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{m{.007\textwidth} m{.10\textwidth} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering}} %{l l cc cc cc cc cc cc cc cc cc}
%     \hline
%   \multirow{2}{*}{\rotatebox{90}{Dataset }} & Poisoning ratio $\rightarrow$ & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}
% \\
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%  & Detection $\downarrow$  & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$  
% \\ 
% \hline \hline 
% \multirow{4}{*}{\rotatebox{90}{ CIFAR10}} & AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% \\ 
%   & SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% \\ 
%   & STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{50.00} & 8.00 & 0.05 
% & \multicolumn{1}{c}{20.00} & 8.15 & 0.05 
% & \multicolumn{1}{c}{44.00} & 8.29 & 0.51  
% & \multicolumn{1}{c}{56.00} & 10.29 & 1.04  
% \\
% \hline
% \multirow{4}{*}{\rotatebox{90}{CIFAR-100}}  &AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 0.97 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.28 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.48 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.92 & 0.00
% \\ 
%   &SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% \\ 
%   &STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.00} & 14.66 & 0.00 
% & \multicolumn{1}{c}{0.00} & 12.56 & 0.00 
% & \multicolumn{1}{c}{48.00} & 13.06 & 0.36  
% & \multicolumn{1}{c}{76.00} & 12.47 & 1.19  
% \\
% \hline

% \multirow{4}{*}{\rotatebox{90}{Tiny ImageNet}}  &AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 1.07 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.68 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.58 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.67 & 0.00
% \\ 
%   &SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% \\ 
%   &STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{25.00} & 15.67 & 0.01 
% & \multicolumn{1}{c}{40.00} & 13.03 & 0.06 
% & \multicolumn{1}{c}{62.00} & 16.16 & 0.38  
% & \multicolumn{1}{c}{78.00} & 15.91 & 0.96  
% \\
% \hline
% \end{tabular}
% }}
% \end{table}
\begin{table}[!ht]
\caption{Results of WPDA against 3 detection methods on PreAct-ResNet18. }
\label{detection_result_pre}
\centering
% \small
% \scriptsize
\normalsize
% \small
\renewcommand{\arraystretch}{1.0}
\scalebox{0.49}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.008\textwidth} m{.07\textwidth} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering}} %{l l cc cc cc cc cc cc cc cc cc}
    % \hline
    \toprule
  \multirow{2}{*}{\rotatebox{90}{ }} & Detection 
  % $\rightarrow$
  & \multicolumn{3}{c}{AC~\cite{chen2018detecting}}        & \multicolumn{3}{c}{SCAn~\cite{tang2021demon} }        & \multicolumn{3}{c}{STRIP~\cite{gao2019strip} }    
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & Poisoning ratio $\downarrow$  & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$   
\\ 
% \hline \hline 
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{CIFAR-10}}} & { 0.004\%}     
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{50.00} & 8.00 & 0.05
\\ 
  & { 0.01\%}
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{20.00} & 8.15 & 0.05  
\\ 
  & { 0.05\%}  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
& \multicolumn{1}{c}{44.00} & 8.29 & 0.51  
\\ 
  & { 0.1\%}  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{56.00} & 10.29 & 1.04  
\\
% \hline
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{CIFAR-100}}} & { 0.004\%}
& \multicolumn{1}{c}{0.00} & 0.97 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 14.66 & 0.00
\\ 
  & {0.01\%}
& \multicolumn{1}{c}{0.00} & 0.28 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 12.56 & 0.00  
\\ 
  & {0.05\%}  
& \multicolumn{1}{c}{0.00} & 0.48 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{48.00} & 13.26 & 0.36  
\\ 
  & {0.1\%}  
& \multicolumn{1}{c}{0.00} & 0.92 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{76.00} & 12.47 & 1.19  
\\
% \hline
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{Tiny ImageNet{}}}}  & {0.004\%}
& \multicolumn{1}{c}{0.00} & 1.07 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{25.00} & 15.67 & 0.01
\\ 
  & {0.01\%}
& \multicolumn{1}{c}{0.00} & 0.68 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{40.00} & 13.03 & 0.06  
\\ 
  & {0.05\%}  
& \multicolumn{1}{c}{0.00} & 0.58 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{62.00} & 16.16 & 0.38  
\\ 
  & {0.1\%}  
& \multicolumn{1}{c}{0.00} & 0.67 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{78.00} & 15.91 & 0.96 
\\
% \hline
\bottomrule
\end{tabular}
}}
\end{table}


==> tables/detection_VGG.tex <==

% \begin{table*}[!ht]
% \caption{The result of WPDA against 3 detection methods under 5 different poisoning ratios in the datasets. The training model adopts VGG19-BN. }
% \label{detection_result_vgg}
% \centering
% % \small
% \normalsize
% \scalebox{0.82}{
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{m{.11\textwidth} m{.1\textwidth} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering}} %{l l cc cc cc cc cc cc cc cc cc}
%     \hline
%   \multirow{2}{*}{Dataset} & Poisoning ratio $\rightarrow$ & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
% \\
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(lr){18-20}
%  & Detection $\downarrow$  & \multicolumn{1}{c}{TPR }    & FPR    & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR    & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR    & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR    & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR    & $F^{\omega}_1$       
% \\ 
% \hline \hline 
% \multirow{4}{*}{CIFAR10} & AC~\cite{chen2018detecting}        
% & \multicolumn{1}{c}{0.00} & 8.42 & 0.00
% & \multicolumn{1}{c}{0.00} & 10.92 & 0.00
% & \multicolumn{1}{c}{0.00} & 11.31 & 0.00
% & \multicolumn{1}{c}{0.00} & 11.31 & 0.00
% & \multicolumn{1}{c}{99.40} & 7.41 & 27.17
% \\ 
%   & SCAn~\cite{tang2021demon}   
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 4.58 & 0.00
% & \multicolumn{1}{c}{98.40} & 0.00 & 93.18  
% \\ 
%   & STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.00} & 10.02 & 0.00 
% & \multicolumn{1}{c}{0.00} & 13.79 & 0.00 
% & \multicolumn{1}{c}{32.00} & 6.64 & 0.46 
% & \multicolumn{1}{c}{42.00} & 8.99 & 0.88  
% & \multicolumn{1}{c}{94.80} & 12.70 & 12.69
% \\
% \hline
% \multirow{4}{*}{CIFAR100} & AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 3.67 & 0.00
% & \multicolumn{1}{c}{0.00} & 3.03 & 0.00
% & \multicolumn{1}{c}{0.00} & 1.24 & 0.00
% & \multicolumn{1}{c}{0.00} & 2.57 & 0.00
% & \multicolumn{1}{c}{0.00} & 2.03 & 0.00
% \\ 
%   & SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% \\ 
%   & STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.00} & 13.65 & 0.00
% & \multicolumn{1}{c}{40.00} & 11.54 & 0.07
% & \multicolumn{1}{c}{52.00} & 19.00 & 0.27  
% & \multicolumn{1}{c}{70.00} & 16.52 & 0.83  
% & \multicolumn{1}{c}{100.00} & 15.10 & 11.80
% \\
% \hline
% \multirow{4}{*}{Tiny ImageNet} & AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 2.98 & 0.00
% & \multicolumn{1}{c}{0.00} & 6.26 & 0.00
% & \multicolumn{1}{c}{0.00} & 7.13 & 0.00
% & \multicolumn{1}{c}{0.00} & 7.98 & 0.00
% & \multicolumn{1}{c}{0.00} & 18.47 & 0.00
% \\ 
%   & SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{99.10} & 0.00 & 96.03 
% \\ 
%   & STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.00} & 16.70 & 0.00 
% & \multicolumn{1}{c}{0.00} & 16.27 & 0.00 
% & \multicolumn{1}{c}{10.00} & 12.88 & 0.08  
% & \multicolumn{1}{c}{9.00} & 13.74 & 0.12  
% & \multicolumn{1}{c}{47.20} & 15.58 & 4.47
% \\
% \hline
% \end{tabular}
% }}
% \end{table*}

\begin{table}[!ht]
\caption{Results of WPDA against 3 detection methods on VGG19-BN. }
\label{detection_result_vgg}
\centering
% \small
% \large
% \scriptsize
\normalsize
% \small
\renewcommand{\arraystretch}{1.0}
\scalebox{0.49}
{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.008\textwidth} m{.07\textwidth} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering} m{.0364\textwidth}<{\centering}} %{l l cc cc cc cc cc cc cc cc cc}
    % \hline
    \toprule 
  \multirow{2}{*}{\rotatebox{90}{ }} & { {Detection}}
  % $\rightarrow$
  & \multicolumn{3}{c}{AC~\cite{chen2018detecting}}        & \multicolumn{3}{c}{SCAn~\cite{tang2021demon} }        & \multicolumn{3}{c}{STRIP~\cite{gao2019strip} }    
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & { {Poisoning ratio}}
 $\downarrow$  
 & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$   
\\ 
% \hline \hline 
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{{CIFAR-10}}}} & { 0.004\%}     
& \multicolumn{1}{c}{0.00} & 8.42 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 10.02 & 0.00
\\ 
  & { 0.01\%}
& \multicolumn{1}{c}{0.00} & 10.92 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 13.79 & 0.00  
\\ 
  & { 0.05\%}  
& \multicolumn{1}{c}{0.00} & 11.31 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{32.00} & 6.64 & 0.46  
\\ 
  & { 0.1\%}  
& \multicolumn{1}{c}{0.00} & 11.31 & 0.00 
& \multicolumn{1}{c}{0.00} & 4.58 & 0.00 
& \multicolumn{1}{c}{42.00} & 8.99 & 0.88  
\\
% \hline
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{CIFAR-100}}} & { 0.004\%}
& \multicolumn{1}{c}{0.00} & 3.67 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 13.65 & 0.00
\\ 
  & {0.01\%}
& \multicolumn{1}{c}{0.00} & 3.03 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{40.00} & 11.54 & 0.07  
\\ 
  & {0.05\%}  
& \multicolumn{1}{c}{0.00} & 1.24 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{52.00} & 19.00 & 0.27  
\\ 
  & {0.1\%}  
& \multicolumn{1}{c}{0.00} & 2.57 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{70.00} & 16.52 & 0.83 
\\
% \hline
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{Tiny ImageNet{}}}}  & {0.004\%}
& \multicolumn{1}{c}{0.00} & 2.98 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 16.70 & 0.00
\\ 
  & {0.01\%}
& \multicolumn{1}{c}{0.00} & 6.26 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 16.27 & 0.00  
\\ 
  & {0.05\%}  
& \multicolumn{1}{c}{0.00} & 7.13 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{10.00} & 12.88 & 0.08  
\\ 
  & {0.1\%}  
& \multicolumn{1}{c}{0.00} & 7.98 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{9.00} & 13.74 & 0.12 
\\
% \hline
\bottomrule
\end{tabular}
}}
\end{table}

==> tables/detection_retrain.tex <==
\begin{table}[!ht]
\caption{The result of 7 compared attack methods and our method under 5 different poisoning ratios in the {CIFAR-100}.}
\label{attack_result_CIFAR-100}
\centering
% \scriptsize
\footnotesize
\scalebox{0.50}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.02\textwidth} m{.1\textwidth} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{0.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering} m{.04\textwidth}<{\centering}} %{l cc cc cc cc cc cc}
    \hline
  \scalebox{0.9}
   { }& {Poisoning ratio $\rightarrow$} & \multicolumn{2}{c}{0.004\%}        & \multicolumn{2}{c}{0.01\%}        & \multicolumn{2}{c}{0.05\%}        & \multicolumn{2}{c}{0.1\%}        & \multicolumn{2}{c}{1\%} 
\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
  &\multicolumn{1}{c}  {Attack $\downarrow$}  & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   
\\ 
\hline \hline 
\multirow{8}{*}{\rotatebox{90}{PreAct-ResNet18}} &  BadNets~\citet{gu2019badnets}     
& \multicolumn{1}{c}{\textbf{70.83}} & 0.13 
& \multicolumn{1}{c}{70.23} & 0.17 
& \multicolumn{1}{c}{70.48} & 0.15 
& \multicolumn{1}{c}{70.80} & 0.20 
& \multicolumn{1}{c}{70.25} & 41.51 
\\ 
& Blended~\citet{chen2017targeted}   
& \multicolumn{1}{c}{70.67} & 0.09  
& \multicolumn{1}{c}{\textbf{70.60}} & 0.34  
& \multicolumn{1}{c}{70.74} & 23.37  
& \multicolumn{1}{c}{70.75} & 52.74 
& \multicolumn{1}{c}{\textbf{70.48}} & 90.67    
\\ 
&\scalebox{0.9}{Input-aware}~\citet{nguyen2020input} 
& \multicolumn{1}{c}{65.27} & 1.11  
& \multicolumn{1}{c}{64.88} & 5.47  
& \multicolumn{1}{c}{62.93} & 39.86  
& \multicolumn{1}{c}{64.18} & 73.11 
& \multicolumn{1}{c}{64.82} & 73.72   
\\ 
&LF~\citet{zeng2021rethinking}     
& \multicolumn{1}{c}{70.72} & 0.10  
& \multicolumn{1}{c}{70.42} & 0.09   
& \multicolumn{1}{c}{\textbf{71.02}} & 0.15 
& \multicolumn{1}{c}{\textbf{70.85}} & 0.84  
& \multicolumn{1}{c}{70.36} & 45.55
\\ 
&SIG~\citet{barni2019new}    
& \multicolumn{1}{c}{70.33} & 0.13  
& \multicolumn{1}{c}{70.38} & 0.52 
& \multicolumn{1}{c}{70.75} & 5.04  
& \multicolumn{1}{c}{70.79} & 11.19  
& \multicolumn{1}{c}{69.81} & 77.85 
\\ 
&SSBA~\citet{li2021invisible}      
& \multicolumn{1}{c}{70.32} & 0.05  
& \multicolumn{1}{c}{70.48} & 0.11 
& \multicolumn{1}{c}{70.64} & 0.15 
& \multicolumn{1}{c}{70.31} & 0.40 
& \multicolumn{1}{c}{70.18} & 44.05
\\ 
&WABA~\citet{drager2022backdoor}  
& \multicolumn{1}{c}{70.18} & 1.29  
& \multicolumn{1}{c}{70.37} & 24.46  
& \multicolumn{1}{c}{70.44} & 71.23 
& \multicolumn{1}{c}{70.28} & 86.48
& \multicolumn{1}{c}{70.42} & \textbf{98.56}
\\ 
% \hline 
&\rowcolor{lightgray!40}{ {WPDA(Ours) }} 
& \multicolumn{1}{c}{ {{{70.28}}}} & { {\textbf{85.01} }}
& \multicolumn{1}{c}{{ {{70.56}}}} & { {\textbf{89.01} }}
& \multicolumn{1}{c}{{ {{70.71}}}} & { {\textbf{95.32}  }}
& \multicolumn{1}{c}{{ {{70.44}}}} & { {\textbf{93.22} }}
& \multicolumn{1}{c}{{ {70.32}}} & { {95.74}}
\\
\hline

\multirow{8}{*}{\rotatebox{90}{VGG19-BN}}  &BadNets~\citet{gu2019badnets}     
& \multicolumn{1}{c}{66.06} & 0.15 
& \multicolumn{1}{c}{65.68} & 0.20 
& \multicolumn{1}{c}{65.64} & 0.23 
& \multicolumn{1}{c}{65.62} & 0.32 
& \multicolumn{1}{c}{65.53} & 69.31 
\\ 
&Blended~\citet{chen2017targeted}   
& \multicolumn{1}{c}{65.34} & 0.07  
& \multicolumn{1}{c}{65.25} & 0.08  
& \multicolumn{1}{c}{65.31} & 14.62  
& \multicolumn{1}{c}{65.65} & 37.05 
& \multicolumn{1}{c}{\textbf{65.57}} & 88.12   
\\ 
&\scalebox{0.9}{Input-aware}~\citet{nguyen2020input} 
& \multicolumn{1}{c}{58.01} & 1.04  
& \multicolumn{1}{c}{57.94} & 1.46  
& \multicolumn{1}{c}{60.37} & 1.00  
& \multicolumn{1}{c}{59.87} & 38.35 
& \multicolumn{1}{c}{59.78} & 36.63   
\\ 
&LF~\citet{zeng2021rethinking}     
& \multicolumn{1}{c}{65.47} & 0.17  
& \multicolumn{1}{c}{\textbf{66.11}} & 0.08   
& \multicolumn{1}{c}{65.59} & 0.25 
& \multicolumn{1}{c}{65.61} & 0.27  
& \multicolumn{1}{c}{65.30} & 0.69 
\\ 
&SIG~\citet{barni2019new}    
& \multicolumn{1}{c}{65.45} & 0.31  
& \multicolumn{1}{c}{65.49} & 0.09 
& \multicolumn{1}{c}{\textbf{65.89}} & 4.60  
& \multicolumn{1}{c}{65.34} & 14.73  
& \multicolumn{1}{c}{65.13} & 72.02 
\\ 
&SSBA~\citet{li2021invisible}      
& \multicolumn{1}{c}{65.56} & 0.09  
& \multicolumn{1}{c}{65.84} & 0.08 
& \multicolumn{1}{c}{66.14} & 0.28 
& \multicolumn{1}{c}{\textbf{65.84}} & 0.52 
& \multicolumn{1}{c}{64.87} & 13.03
\\ 
&WABA~\citet{drager2022backdoor}  
& \multicolumn{1}{c}{65.40} & 0.40  
& \multicolumn{1}{c}{65.57} & 7.61  
& \multicolumn{1}{c}{65.48} & 65.72 
& \multicolumn{1}{c}{66.20} & 85.47    
& \multicolumn{1}{c}{65.59} & \textbf{97.64}
\\ 
% \hline 
& \rowcolor{lightgray!40} {WPDA(Ours)} 
& \multicolumn{1}{c}
 { {\textbf{66.24}}} & 
{ {\textbf{79.94}  }}
& \multicolumn{1}{c}{ {65.18}} & 
{ {\textbf{88.09} }}
& \multicolumn{1}{c}{ {65.62}} & 
{ {\textbf{97.20}  } }
& \multicolumn{1}{c}{ {65.47}} & 
{ {\textbf{91.06}  }}
& \multicolumn{1}{c}{ {{65.13}}} & 
{ {{94.58}}}  
\\
\hline
\end{tabular}
}}
\end{table}

==> tables/experiment_attack_cifar100_new.tex <==
\begin{table}[!ht]
\caption{Results of 7 compared attack methods and our method on the {CIFAR-100}.}
\label{attack_result_CIFAR-100}
\centering
% \normalsize
\small
\scalebox{0.49}
{
\resizebox{\textwidth}{!}{
    \begin{tabular}
    {m{.002\textwidth} m{.09\textwidth} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} }  %{l cc cc cc cc cc cc}
    \toprule
   { }& {Poisoning {} ratio} & \multicolumn{2}{c}{0.004\%}        & \multicolumn{2}{c}{0.01\%}        & \multicolumn{2}{c}{0.05\%}        & \multicolumn{2}{c}{0.1\%}        
\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}  
  &\multicolumn{1}{c}  {Attack $\downarrow$}  & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR  
\\ 
% \hline
\midrule
% \hline 
\multirow{8}{*}{\rotatebox{90}{PreAct-ResNet18}} &  BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{\textbf{70.83}} & 0.13 
& \multicolumn{1}{c}{70.23} & 0.17 
& \multicolumn{1}{c}{70.48} & 0.15 
& \multicolumn{1}{c}{70.80} & 0.20 
\\ 
& Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{70.67} & 0.09  
& \multicolumn{1}{c}{\textbf{70.60}} & 0.34  
& \multicolumn{1}{c}{70.74} & 23.37  
& \multicolumn{1}{c}{70.75} & 52.74    
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{65.27} & 1.11  
& \multicolumn{1}{c}{64.88} & 5.47  
& \multicolumn{1}{c}{62.93} & 39.86  
& \multicolumn{1}{c}{64.18} & 73.11 
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{70.72} & 0.10  
& \multicolumn{1}{c}{70.42} & 0.09   
& \multicolumn{1}{c}{\textbf{71.02}} & 0.15 
& \multicolumn{1}{c}{\textbf{70.85}} & 0.84  
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{70.33} & 0.13  
& \multicolumn{1}{c}{70.38} & 0.52 
& \multicolumn{1}{c}{70.75} & 5.04  
& \multicolumn{1}{c}{70.79} & 11.19  
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{70.32} & 0.05  
& \multicolumn{1}{c}{70.48} & 0.11 
& \multicolumn{1}{c}{70.64} & 0.15 
& \multicolumn{1}{c}{70.31} & 0.40 
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{70.18} & 1.29  
& \multicolumn{1}{c}{70.37} & 24.46  
& \multicolumn{1}{c}{70.44} & 71.23 
& \multicolumn{1}{c}{70.28} & 86.48
\\ 
% \hline 
\rowcolor{lightgray!40}& {WPDA(Ours)}  
& \multicolumn{1}{c}{ {{{70.28}}}} & { {\textbf{85.01} }}
& \multicolumn{1}{c}{{ {{70.56}}}} & { {\textbf{89.01} }}
& \multicolumn{1}{c}{{ {{70.71}}}} & { {\textbf{95.32}  }}
& \multicolumn{1}{c}{{ {{70.44}}}} & { {\textbf{93.22} }}
\\
% \hline
\midrule
\multirow{8}{*}{\rotatebox{90}{VGG19-BN}}  &BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{66.06} & 0.15 
& \multicolumn{1}{c}{65.68} & 0.20 
& \multicolumn{1}{c}{65.64} & 0.23 
& \multicolumn{1}{c}{65.62} & 0.32 
\\ 
&Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{65.34} & 0.07  
& \multicolumn{1}{c}{65.25} & 0.08  
& \multicolumn{1}{c}{65.31} & 14.62  
& \multicolumn{1}{c}{65.65} & 37.05  
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{58.01} & 1.04  
& \multicolumn{1}{c}{57.94} & 1.46  
& \multicolumn{1}{c}{60.37} & 1.00  
& \multicolumn{1}{c}{59.87} & 38.35
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{65.47} & 0.17  
& \multicolumn{1}{c}{\textbf{66.11}} & 0.08   
& \multicolumn{1}{c}{65.59} & 0.25 
& \multicolumn{1}{c}{65.61} & 0.27  
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{65.45} & 0.31  
& \multicolumn{1}{c}{65.49} & 0.09 
& \multicolumn{1}{c}{\textbf{65.89}} & 4.60  
& \multicolumn{1}{c}{65.34} & 14.73  
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{65.56} & 0.09  
& \multicolumn{1}{c}{65.84} & 0.08 
& \multicolumn{1}{c}{66.14} & 0.28 
& \multicolumn{1}{c}{\textbf{65.84}} & 0.52 
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{65.40} & 0.40  
& \multicolumn{1}{c}{65.57} & 7.61  
& \multicolumn{1}{c}{65.48} & 65.72 
& \multicolumn{1}{c}{66.20} & 85.47    
\\ 
% \hline 
\rowcolor{lightgray!40}& {WPDA(Ours)}  
& \multicolumn{1}{c}
 {{\textbf{66.24}}} & 
{{\textbf{79.94}  }}
& \multicolumn{1}{c}{{65.18}} & 
{{\textbf{88.09} }}
& \multicolumn{1}{c}{{65.62}} & 
{{\textbf{97.20}}}
& \multicolumn{1}{c}{{65.47}} & 
{{\textbf{91.06}}}
\\
\bottomrule
\end{tabular}
}} 
\end{table}


==> tables/experiment_attack_cifar10_new.tex <==
\begin{table}[!ht]
\caption{Results of 7 compared attack methods and our method on the CIFAR-10.}
\label{attack_result_CIFAR-10}
\centering
% \scriptsize
% %\footnotesize
% \tiny
% \normalsize
\small
\scalebox{0.49}
{
\resizebox{\textwidth}{!}{
    \begin{tabular}
    {m{.002\textwidth} m{.09\textwidth} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} } 

    \toprule
   { }& {Poisoning {}ratio } & \multicolumn{2}{c}{0.004\%}        & \multicolumn{2}{c}{0.01\%}        & \multicolumn{2}{c}{0.05\%}        & \multicolumn{2}{c}{0.1\%}        
\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} 
  &\multicolumn{1}{c}  {Attack $\downarrow$}  & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   
\\ 
% \hline 
\midrule
% \hline 
\multirow{8}{*}{\rotatebox{90}{{PreAct-ResNet18}}} &  BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{93.68} & 0.67 
& \multicolumn{1}{c}{93.74} & 0.88 
& \multicolumn{1}{c}{93.70} & 0.72 
& \multicolumn{1}{c}{93.61} & 1.23 
% & \multicolumn{1}{c}{93.14} & 74.73 
\\ 
& Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{94.21} & 4.81  
& \multicolumn{1}{c}{94.00} & 7.49  
& \multicolumn{1}{c}{93.81} & 26.07  
& \multicolumn{1}{c}{93.80} & 56.11 
% & \multicolumn{1}{c}{93.76} & 94.88   
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{91.54} & 12.36  
& \multicolumn{1}{c}{90.28} & 13.73  
& \multicolumn{1}{c}{90.66} & 38.78  
& \multicolumn{1}{c}{91.94} & 47.32 
% & \multicolumn{1}{c}{91.74} & 79.18   
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{93.93} & 0.94  
& \multicolumn{1}{c}{\textbf{93.98}} & 1.22   
& \multicolumn{1}{c}{\textbf{94.06}} & 1.39 
& \multicolumn{1}{c}{93.55} & 12.72  
% & \multicolumn{1}{c}{93.56} & 86.46
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{93.94} & 0.53  
& \multicolumn{1}{c}{93.75} & 1.07 
& \multicolumn{1}{c}{93.93} & 18.76  
& \multicolumn{1}{c}{\textbf{94.05}} & 54.88  
% & \multicolumn{1}{c}{93.68} & 87.71 
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{93.81} & 0.71  
& \multicolumn{1}{c}{94.10} & 0.59 
& \multicolumn{1}{c}{93.90} & 1.27 
& \multicolumn{1}{c}{93.89} & 1.62 
% & \multicolumn{1}{c}{93.43} & 73.44
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{93.95} & 5.87  
& \multicolumn{1}{c}{93.76} & 10.62  
& \multicolumn{1}{c}{93.67} & 68.09 
& \multicolumn{1}{c}{93.77} & 86.16
% & \multicolumn{1}{c}{93.65} & 99.19 
\\ 

\rowcolor{lightgray!40} & WPDA(Ours)  
& \multicolumn{1}{c}{ {{\textbf{94.03}}}} & { {\textbf{98.12}  }}
& \multicolumn{1}{c}{{ {{93.89}}}} & { {\textbf{98.71} }}
& \multicolumn{1}{c}{{ {{93.58}}}} & { {\textbf{99.80}  }}
& \multicolumn{1}{c}{{ {{93.84}}}} & { {\textbf{99.76} }}
% & \multicolumn{1}{c}{{ {\textbf{93.86}}}} & { {\textbf{100.00}}}
\\

% \hline
\midrule
\multirow{8}{*}{\rotatebox{90}{{VGG19-BN}}}  &BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{92.23} & 0.89 
& \multicolumn{1}{c}{91.96} & 0.82 
& \multicolumn{1}{c}{92.23} & 0.94 
& \multicolumn{1}{c}{92.03} & 1.09 
% & \multicolumn{1}{c}{91.73} & 74.66 
\\ 
&Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{92.25} & 3.41  
& \multicolumn{1}{c}{91.73} & 5.67  
& \multicolumn{1}{c}{92.32} & 22.24  
& \multicolumn{1}{c}{92.16} & 44.10 
% & \multicolumn{1}{c}{92.06} & 92.87   
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{89.47} & 10.19  
& \multicolumn{1}{c}{89.40} & 11.89  
& \multicolumn{1}{c}{89.62} & 59.82  
& \multicolumn{1}{c}{89.36} & 77.16 
% & \multicolumn{1}{c}{89.02} & 67.30   
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{92.12} & 2.30  
& \multicolumn{1}{c}{\textbf{92.43}} & 0.76   
& \multicolumn{1}{c}{91.94} & 0.97 
& \multicolumn{1}{c}{92.21} & 0.92  
% & \multicolumn{1}{c}{91.41} & 1.89 
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{92.14} & 0.73  
& \multicolumn{1}{c}{91.97} & 2.31 
& \multicolumn{1}{c}{92.20} & 12.47  
& \multicolumn{1}{c}{91.96} & 33.74  
% & \multicolumn{1}{c}{92.03} & 91.06 
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{92.26} & 0.98  
& \multicolumn{1}{c}{92.33} & 0.97 
& \multicolumn{1}{c}{\textbf{92.38}} & 1.21 
& \multicolumn{1}{c}{92.36} & 1.44 
% & \multicolumn{1}{c}{91.94} & 38.39
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{92.08} & 3.03  
& \multicolumn{1}{c}{92.02} & 20.74  
& \multicolumn{1}{c}{91.91} & 48.09 
& \multicolumn{1}{c}{91.87} & 79.13 
% & \multicolumn{1}{c}{\textbf{92.27}} & 97.93 
\\ 
% \hline 
\rowcolor{lightgray!40}& {WPDA(Ours)}  
& \multicolumn{1}{c}{{{\textbf{92.49}}}} & {{\textbf{77.50}}}
& \multicolumn{1}{c}{{92.29}} & {{\textbf{91.79}}}
& \multicolumn{1}{c}{{92.33}} & {{\textbf{99.23}}}
& \multicolumn{1}{c}{{\textbf{92.50}}} & {{\textbf{99.64}}}
% & \multicolumn{1}{c}{ {{92.01}}} & { {\textbf{99.99}}}
\\
\bottomrule
\end{tabular}
}}
\end{table}


==> tables/experiment_attack_tiny_new.tex <==
\begin{table}[!ht]
\caption{Results of 7 compared attack methods and our method on the {Tiny ImageNet}.}
\label{attack_result_tiny}
\centering
% \scriptsize
% \normalsize
\small
\scalebox{0.49}{
\resizebox{\textwidth}{!}{
    \begin{tabular}
    {m{.002\textwidth} m{.09\textwidth} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} m{.036\textwidth}<{\centering} } %{l cc cc cc cc cc cc}
    \toprule
   { }& {Poisoning {}ratio } & \multicolumn{2}{c}{0.004\%}        & \multicolumn{2}{c}{0.01\%}        & \multicolumn{2}{c}{0.05\%}        & \multicolumn{2}{c}{0.1\%}            
\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} 
  &\multicolumn{1}{c}  {Attack $\downarrow$}  & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR   & \multicolumn{1}{c}{C-Acc}    & ASR       
\\ 
% \hline 
\midrule
% \hline 
\multirow{8}{*}{\rotatebox{90}{PreAct-ResNet18}} &  BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{56.87} & 0.12 
& \multicolumn{1}{c}{56.86} & 0.18 
& \multicolumn{1}{c}{57.26} & 0.25 
& \multicolumn{1}{c}{57.51} & 33.53 
% & \multicolumn{1}{c}{57.51} & 95.01 
\\ 
& Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{57.24} & 0.06  
& \multicolumn{1}{c}{57.11} & 2.90  
& \multicolumn{1}{c}{57.68} & 50.88  
& \multicolumn{1}{c}{57.58} & 65.19 
% & \multicolumn{1}{c}{{57.31}} & 95.29   
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{\textbf{58.55}} & 2.00   
& \multicolumn{1}{c}{\textbf{57.93}} & 34.96  
& \multicolumn{1}{c}{\textbf{58.05}} & 57.29  
& \multicolumn{1}{c}{\textbf{57.96}} & 63.80 
% & \multicolumn{1}{c}{\textbf{57.94}} & 85.12   
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{56.98} & 0.17  
& \multicolumn{1}{c}{57.03} & 0.13   
& \multicolumn{1}{c}{{57.26}} & 0.16 
& \multicolumn{1}{c}{{56.97}} & 19.49  
% & \multicolumn{1}{c}{56.47} & 83.03
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{57.11} & 4.14  
& \multicolumn{1}{c}{57.16} & 10.32 
& \multicolumn{1}{c}{56.86} & 27.42  
& \multicolumn{1}{c}{57.03} & 44.93  
% & \multicolumn{1}{c}{---} & --- 
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{56.80} & 0.11  
& \multicolumn{1}{c}{56.96} & 0.30 
& \multicolumn{1}{c}{57.23} & 2.31 
& \multicolumn{1}{c}{57.20} & 13.28 
% & \multicolumn{1}{c}{56.88} & 80.43
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{57.10} & 4.13  
& \multicolumn{1}{c}{57.30} & 15.92  
& \multicolumn{1}{c}{56.51} & 74.14
& \multicolumn{1}{c}{57.17} & 90.13
% & \multicolumn{1}{c}{56.82} & {98.37}
\\ 
% \hline 
\rowcolor{lightgray!40}& {WPDA(Ours)}  
& \multicolumn{1}{c}{{{57.24}}} & {{\textbf{80.99} }}
& \multicolumn{1}{c}{{{{56.88}}}} & {{\textbf{85.80}  }}
& \multicolumn{1}{c}{{{{56.73}}}} & {{\textbf{88.45} }}
& \multicolumn{1}{c}{{{{56.86}}}} & {{\textbf{90.71}}}
% & \multicolumn{1}{c}{{{57.28}}} & {{\textbf{98.53}}}
\\
% \hline
\midrule
\multirow{8}{*}{\rotatebox{90}{VGG19-BN}}  &BadNets~\cite{gu2019badnets}     
& \multicolumn{1}{c}{53.65} & 0.24 
& \multicolumn{1}{c}{53.99} & 0.18 
& \multicolumn{1}{c}{53.87} & 0.38 
& \multicolumn{1}{c}{54.85} & 48.85 
% & \multicolumn{1}{c}{53.48} & \textbf{98.86}
\\ 
&Blended~\cite{chen2017targeted}   
& \multicolumn{1}{c}{53.77} & 0.23 
& \multicolumn{1}{c}{53.71} & 5.88  
& \multicolumn{1}{c}{53.53} & 52.88  
& \multicolumn{1}{c}{53.43} & 69.38 
% & \multicolumn{1}{c}{{52.47}} & 94.90   
\\ 
&\scalebox{0.9}{Input-aware}~\cite{nguyen2020input} 
& \multicolumn{1}{c}{53.80} & 8.91   
& \multicolumn{1}{c}{53.98} & 17.71  
& \multicolumn{1}{c}{53.92} & 35.13  
& \multicolumn{1}{c}{\textbf{54.09}} & 85.43 
% & \multicolumn{1}{c}{\textbf{54.10}} & 79.82   
\\ 
&LF~\cite{zeng2021rethinking}     
& \multicolumn{1}{c}{54.02} & 0.16  
& \multicolumn{1}{c}{53.28} & 0.17   
& \multicolumn{1}{c}{{53.25}} & 0.22 
& \multicolumn{1}{c}{{52.80}} & 0.22  
% & \multicolumn{1}{c}{51.94} & 0.51
\\ 
&SIG~\cite{barni2019new}    
& \multicolumn{1}{c}{53.35} & 3.09 
& \multicolumn{1}{c}{54.24} & 1.65 
& \multicolumn{1}{c}{53.62} & 12.41  
& \multicolumn{1}{c}{53.33} & 26.92  
% & \multicolumn{1}{c}{---} & --- 
\\ 
&SSBA~\cite{li2021invisible}      
& \multicolumn{1}{c}{\textbf{54.15}} & 0.02  
& \multicolumn{1}{c}{53.17} & 0.22 
& \multicolumn{1}{c}{\textbf{54.35}} & 2.42 
& \multicolumn{1}{c}{53.91} & 8.42 
% & \multicolumn{1}{c}{53.10} & 86.63
\\ 
&WABA~\cite{drager2022backdoor}  
& \multicolumn{1}{c}{52.43} & 9.76  
& \multicolumn{1}{c}{53.20} & 24.90  
& \multicolumn{1}{c}{53.80} & 80.37
& \multicolumn{1}{c}{53.80} & 93.40
% & \multicolumn{1}{c}{{53.22}} & {98.50}
\\ 
% \hline 
\rowcolor{lightgray!40}& {WPDA(Ours)}  
& \multicolumn{1}{c}{{{{53.46}}}} & {{\textbf{64.96}}}
& \multicolumn{1}{c}{{\textbf{54.25}}} & {{\textbf{81.89}}}
& \multicolumn{1}{c}{{53.74}} & {{\textbf{91.96}}}
& \multicolumn{1}{c}{{53.99}} & {{\textbf{90.30}}}
% & \multicolumn{1}{c}{{{51.39}}} & {{{96.03}}}
\\
\bottomrule
\end{tabular}
}}
\end{table}

==> tables/experiment_detection1.tex <==
\begin{table*}[!ht]
\caption{The result of WPDA against 3 detection methods under 5 different poisoning ratios in the datasets. The training model adopts PreAct-ResNet18. }
\label{detection_result_pre}
\centering
% \small
% \large
\normalsize
\scalebox{0.82}{
\resizebox{\textwidth}{!}{
    \begin{tabular}{m{.11\textwidth} m{.1\textwidth} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering} m{.0355\textwidth}<{\centering}} %{l l cc cc cc cc cc cc cc cc cc}
    \toprule
  \multirow{2}{*}{Dataset} & Poisoning ratio $\rightarrow$ & \multicolumn{3}{c}{0.004\%}        & \multicolumn{3}{c}{0.01\%}        & \multicolumn{3}{c}{0.05\%}        & \multicolumn{3}{c}{0.1\%}        & \multicolumn{3}{c}{1\%} 
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} \cmidrule(lr){18-20}
 & Detection $\downarrow$  & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$    & \multicolumn{1}{c}{TPR }    & FPR     & $F^{\omega}_1$       
\\ 
\hline \hline 
\multirow{4}{*}{CIFAR10} & AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
\\ 
  & SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
\\ 
%   & Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
% & \multicolumn{1}{c}{0.12} & 0.15 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00
%   & Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{0.00} & 15.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 15.00 & 0.00 
% & \multicolumn{1}{c}{12.00} & 15.01 & 0.08  
% & \multicolumn{1}{c}{0.00} & 15.02 & 0.00  
% & \multicolumn{1}{c}{0.00} & 15.16 & 0.00
% \\ 
  & STRIP~\cite{gao2019strip}    
& \multicolumn{1}{c}{50.00} & 8.00 & 0.05 
& \multicolumn{1}{c}{20.00} & 8.15 & 0.05 
& \multicolumn{1}{c}{44.00} & 8.29 & 0.51  
& \multicolumn{1}{c}{56.00} & 10.29 & 1.04  
& \multicolumn{1}{c}{93.80} & 12.25 & 12.88
\\
\hline
% \multirow{4}{*}{CIFAR-100}  &AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 0.04 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.03 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.01 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.03 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.02 & 0.00
% \\ 
%   &SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% \\ 
%   &Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{1.00} & 0.15 & 0.00 
% & \multicolumn{1}{c}{1.00} & 0.15 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00  
% & \multicolumn{1}{c}{1.00} & 0.15 & 0.01  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00
% \\ 
%   &STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.00} & 0.12 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.13 & 0.00 
% & \multicolumn{1}{c}{0.48} & 0.13 & 0.00  
% & \multicolumn{1}{c}{0.78} & 0.13 & 0.01  
% & \multicolumn{1}{c}{1.00} & 0.13 & 0.14
\multirow{4}{*}{CIFAR-100}  &AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 0.97 & 0.00
& \multicolumn{1}{c}{0.00} & 0.28 & 0.00
& \multicolumn{1}{c}{0.00} & 0.48 & 0.00
& \multicolumn{1}{c}{0.00} & 0.92 & 0.00
& \multicolumn{1}{c}{0.00} & 0.93 & 0.00
\\ 
  &SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% \\ 
%   &Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{100.00} & 30.00 & 0.03 
% & \multicolumn{1}{c}{100.00} & 30.00 & 0.07 
% & \multicolumn{1}{c}{0.00} & 15.02 & 0.00  
% & \multicolumn{1}{c}{100.00} & 30.00 & 0.66 
% & \multicolumn{1}{c}{0.00} & 15.22 & 0.00
\\ 
  &STRIP~\cite{gao2019strip}    
& \multicolumn{1}{c}{0.00} & 14.66 & 0.00 
& \multicolumn{1}{c}{0.00} & 12.56 & 0.00 
& \multicolumn{1}{c}{48.00} & 13.06 & 0.36  
& \multicolumn{1}{c}{76.00} & 12.47 & 1.19  
& \multicolumn{1}{c}{100.00} & 8.31 & 19.56
\\
\hline
% \multirow{4}{*}{Tiny ImageNet}  &AC~\cite{chen2018detecting}     
% & \multicolumn{1}{c}{0.00} & 0.01 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.01 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.01 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.01 & 0.00
% & \multicolumn{1}{c}{0.00} & 0.02 & 0.00
% \\ 
%   &SCAn~\cite{tang2021demon} 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{0.99} & 0.00 & 0.96
% & \multicolumn{1}{c}{0.99} & 0.00 & 1.00  
% \\ 
%   &Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00 
% & \multicolumn{1}{c}{0.70} & 0.00 & 0.14 
% & \multicolumn{1}{c}{0.40} & 0.15 & 0.00  
% & \multicolumn{1}{c}{0.80} & 0.15 & 0.01  
% & \multicolumn{1}{c}{0.00} & 0.15 & 0.00
% \\ 
%   &STRIP~\cite{gao2019strip}    
% & \multicolumn{1}{c}{0.25} & 0.16 & 0.00 
% & \multicolumn{1}{c}{0.40} & 0.13 & 0.00 
% & \multicolumn{1}{c}{0.62} & 0.16 & 0.00  
% & \multicolumn{1}{c}{0.78} & 0.16 & 0.01  
% & \multicolumn{1}{c}{0.96} & 0.18 & 0.10
\multirow{4}{*}{Tiny ImageNet}  &AC~\cite{chen2018detecting}     
& \multicolumn{1}{c}{0.00} & 1.07 & 0.00
& \multicolumn{1}{c}{0.00} & 0.68 & 0.00
& \multicolumn{1}{c}{0.00} & 0.58 & 0.00
& \multicolumn{1}{c}{0.00} & 0.67 & 0.00
& \multicolumn{1}{c}{0.00} & 1.60 & 0.00
\\ 
  &SCAn~\cite{tang2021demon} 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00 
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
& \multicolumn{1}{c}{0.00} & 0.00 & 0.00  
% & \multicolumn{1}{c}{99.00} & 0.00 & 95.65
& \multicolumn{1}{c}{99.90} & 0.00 & 99.50  
% \\ 
%   &Spectral~\cite{tran2018spectral}  
% & \multicolumn{1}{c}{0.00} & 15.00 & 0.00 
% & \multicolumn{1}{c}{90.00} & 14.99 & 0.12 
% & \multicolumn{1}{c}{40.00} & 15.00 & 0.26  
% & \multicolumn{1}{c}{80.00} & 14.95 & 1.05  
% & \multicolumn{1}{c}{0.00} & 15.22 & 0.00
\\ 
  &STRIP~\cite{gao2019strip}    
& \multicolumn{1}{c}{25.00} & 15.67 & 0.01 
& \multicolumn{1}{c}{40.00} & 13.03 & 0.06 
& \multicolumn{1}{c}{62.00} & 16.16 & 0.38  
& \multicolumn{1}{c}{78.00} & 15.91 & 0.96  
& \multicolumn{1}{c}{95.70} & 18.41 & 9.32
\\
\bottomrule
\end{tabular}
}}
\end{table*}


==> tables/image_quality.tex <==
\begin{table}[!ht]
\centering
\caption{Quality of test samples generated by 8 attack methods at 0.004\% poisoning ratio.}
% \scriptsize
% \resizebox{\columnwidth}{!}
{
\label{image_quality}
\scalebox{0.95}{
\begin{tabular}{ccccccccc}
\hline 
Metric & BadNets & Blended & Input-aware & LF    & SIG   & SSBA  & WABA  & WPDA(ours)  \\ \hline \hline
SSIM   & 0.999   & 0.792   & 0.899       & 0.987 & 0.604 & 0.882 & 0.643 & 0.665 \\ \hline
MSE    & 0.095   & 0.288   & 0.176       & 0.053 & 0.371 & 0.122 & 1.063 & 0.404 \\ \hline
\end{tabular}
}}
\end{table}

==> tables/notation1.tex <==

\begin{table*}[ht]
\caption{Notation definitions.}
\renewcommand\arraystretch{1.1}
\centering
\setlength{\tabcolsep}{2pt}
\scalebox{0.9}{
\begin{tabular}{c|l}
\toprule
Notation  &  Definition  
\\ 
\hline
$\x$  & One data point, vector  
\\ 
$y$  &  One label, scalar  
\\ 
$f_{\btheta}$  &  Model with parameter
\\ 
$\btheta$  &  Model parameters  
\\ 
$f_{\btheta}(\x)$ & Model output
\\
$\mathcal{X} \in \mathbb{R}^3$  & $3$-dimensional input space 
\\
$\mathcal{Y} \in \{1, 2, \ldots, C\}$ & Output space with $C$ candidate classes
\\
$\D = \{(\x^{(i)}, y^{(i)})\}_{i=1}^n$  &  Dataset with $n$ samples 
\\ 
$\hat{\D}_p = \{(\hat{\x}^{(i)}, t) | (\x^{(i)}, y^{(i)}) \in \D_p \})$  & Set of poisoned sample pairs  
\\ 
$\hat{\D} = \{\D_c, \hat{\D}_p\}$  & Poisoned
training dataset 
\\
$p = \frac{|\hat{\D}_p|}{|\hat{\D}|}$  & Poisoning ratio 
\\
$\triangle$  & Trigger image in spatial domain 
\\
$\triangle_{fre}$  & Trigger image in frequency domain 
\\
$N$  & Level of WPD 
\\
$\mathcal W^{N}(\cdot)$  & $N$-level WPD
\\
$C^N_{s,p}=\mathcal W^{N}_{s,p}(\cdot)$  & \multicolumn{1}{l}{A coefficient matrix representing the $s$-th sub-spectrogram }\\& \multicolumn{1}{l}{in the $p$-th parent-spectrogram}
\\
$\mathcal W^{-N}(\cdot)$  & $N$-level IWPD
\\
$\mathcal{T}$  & Average transformation
training dataset 
\\
$\mathbf{m} \in \left \{ 0,1 \right \} ^{(M+2L) \times (M+2L) \times 3}$  & A binary mask with the shape of ${(M+2L) \times (M+2L) \times 3}$
\\
$2L$  & The vanishing moment of the wavelet basis function
\\
$\odot$  & Element-wise multiplication of matrices
\\
$k$  & The intensity of the trigger image information $\triangle_{fre}$ in the poisoned training samples $\hat{\boldsymbol{x}}_{train}$
\\
$k'$  & The intensity of the trigger image information $\triangle_{fre}$ in the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$
\\
$\alpha$  & \multicolumn{1}{l}{The intensity of the original benign sample information in} \\& \multicolumn{1}{l}{the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$}
\\
\bottomrule
\end{tabular}%
}
\label{table: template}
\end{table*}





==> tip/1_abstract_keywords.tex <==
\begin{abstract}
This work explores backdoor attack, an emerging security threat against deep neural networks (DNNs). The adversary aims to inject a backdoor into the model by manipulating a small portion of the training data, such that the backdoor could be activated by a particular trigger and bootstraps the model to make a target prediction at inference. Currently, most existing data-poisoning based attacks often struggle with maintaining efficacy at low poisoning ratios, making them susceptible to defense techniques. To address this challenge, we propose a novel frequency-based backdoor attack via Wavelet Packet Decomposition (WPD), an advanced signal processing technique that decomposes the original image signal into a spectrogram and captures frequency information with semantic meanings. Specifically, we leverage WPD to statistically analyze the frequency distribution of the dataset to identify the key frequency regions the DNNs would focus on, then the trigger information is only injected into such key frequency regions. Our method mainly includes three parts: 1) selecting the poisoning frequency regions in spectrogram; 2) crafting the trigger; 3) constructing the poisoned dataset. Our method stands out for its exceptional stealth and precision, as evidenced by achieving the $98.12\%$ Attack Success Rate (ASR) on CIFAR-10 with the extremely low poisoning ratio $0.004\%$ (\textit{i.e.}, only 2 poisoned samples among 50,000 training samples) and bypassing most existing defense methods. Besides, we also provide visualization analyses to explain the underlying mechanism.



\end{abstract}
\begin{IEEEkeywords}
Backdoor attack, wavelet packet transform, low poisoning ratios
\end{IEEEkeywords}




% \begin{abstract}
% This work explores backdoor attack, an emerging security threat against deep neural networks (DNNs). The adversary aims to inject a backdoor into the model by manipulating a portion of the training data, such that the backdoor could be activated by a particular trigger and bootstraps the model to make a target prediction at inference. Currently, most existing data-poisoning based attacks often struggle with maintaining efficacy at low poisoning ratios, making them susceptible to defense techniques. To address this challenge, we propose a novel frequency-based backdoor attack via Wavelet Packet Decomposition (WPD), an advanced signal processing technique that decomposes the original image signal into a spectrogram and captures frequency information with semantic meanings. Specifically, we leverage WPD to statistically analyze the frequency distribution of the dataset to identify the key frequency regions the DNNs would focus on, then the trigger information is only injected into such key frequency regions. Our method mainly includes three parts: 1) selecting the poisoning frequency regions in spectrogram; 2) crafting the trigger; 3) constructing the poisoned dataset. Our method stands out for its exceptional stealth and precision, as evidenced by achieving the $98.12\%$ Attack Success Rate (ASR) on CIFAR-10 with an extremely low poisoning ratio of $0.004\%$ (\textit{i.e.}, only 2 poisoned samples among 50,000 training samples) and bypassing most existing defense methods. Besides, we also provide comprehensive experiments and analyses to explain the underlying mechanism.

% \end{abstract}
% \begin{IEEEkeywords}
% Backdoor attack, wavelet packet transform, low poisoning ratios
% \end{IEEEkeywords}

==> tip/2_Introduction.tex <==
\section{Introduction}
\IEEEPARstart{D}{eep}
neural networks (DNNs) have achieved remarkable success and widespread adoption in various research fields (\eg, face recognition~\cite{balaban2015deep,Wei_Adversarial2023}, voice recognition~\cite{li2012improving,yuan2018commandersong}, and autonomous driving~\cite{zhou2020deepbillboard}), leading to significant advancements in artificial intelligence. However, this progress also introduces potential security vulnerabilities. 
Among these security threats, backdoor attacks pose a significant risk, involving maliciously manipulating a DNN model during training to embed hidden backdoors. These backdoors can be triggered by specific input patterns, causing the model to produce targeted incorrect outputs while maintaining normal performance on benign inputs. The implications of such attacks range from targeted misclassification and data manipulation to compromising the integrity and reliability of critical systems that rely on DNNs.

In this work, we study the threat model of data poisoning- based backdoor attack, where the attack can only manipulate the training dataset, without access to the training process. It applies to the practical scenario that the user doesn't have sufficient training data, thus download or buy data from an untrustworthy third-party data platform. Although several effective backdoor attacks have been developed, they often require a substantial number of poisoned training samples to achieve the desired attack success rate, potentially increasing the risk of being detected by detection methods or defended by defense methods. Our goal is to achieve a precious attack at low poisoning ratios, which is necessary and challenging~\cite{wu2022backdoorbench}. 
% so it is necessary to find out a stable and stealthy backdoor attack method in the setting of low poisoning ratios~\cite{wubackdoorbench}. However, it is very challenging to achieve a high attack success rate while maintaining the naturalness of the poisoned samples. 

% Instead of searching the key region in the original spatial domain of the image, 
% Poisoned samples generated by the spacial domain-based backdoor attacks usually have anomalous pixels.
% Low-poisoning backdoor attacks present a key challenge: enabling models to learn the trigger from limited poisoned samples. To overcome this, we propose first identifying the data regions that models prioritize during training, then strategically embedding the trigger within these regions for optimal effectiveness.
In scenarios of backdoor attacks with a low poisoning ratio, the primary challenge is ensuring that the model can effectively learn the trigger from a limited number of poisoned training samples. 
\textit{The key to overcoming this challenge lies in inferring the important regions of datasets information that the models focus on during the training process and strategically injecting the trigger into these regions.
% We believe that effectively overcoming this challenge involves first inferring the regions of important datasets information that models focus on during training process, and then strategically injecting the trigger into the corresponding regions. 
% Low-poisoning backdoor attacks exist a key challenge: enabling models to learn the trigger from limited poisoned samples. To overcome this, we propose first inferring the important datasets information regions that models focus on during training process, and then strategically injecting the trigger into the corresponding regions. 
}
Compared to the spatial domain, backdoor attacks based on the frequency domain are more adept at preserving the naturalness of backdoor samples. Considering the design of subsequent methods, we analyze the distribution of datasets information in the frequency domain space. Currently, several techniques exist for transforming an image from spatial space to frequency space, including the Discrete Cosine Transform (DCT)~\cite{ahmed1974discrete}, Discrete Fourier Transform (DFT)~\cite{winograd1978computing}, and Wavelet Packet Decomposition (WPD)~\cite{xiong1998wavelet}. 
Among these methods, WPD provides a unique multi-scale frequency domain analysis, effectively capturing features of images at various scales. This analysis not only enhances our overall understanding of the image's structural compositions but also makes WPD particularly adept at precisely locating and representing local image features with distinct semantic meanings within the frequency domain. Consequently, WPD facilitates a more detailed analysis of frequency information distribution within the dataset, enabling us to select key frequency regions in the spectrogram for trigger injection to achieve successful backdoor attacks at low poisoning ratios.
% The poisoned samples generated by spatial domain-based backdoor attacks, which can achieve success at low poisoning ratios, usually tend to have anomalous pixels. To tackle this issue, we propose to explore in the frequency domain. Frequency domain-based backdoor attacks can perform more granular manipulations on specific parts of the image, and it is also easier to maintain the naturalness of the image. Currently, several techniques exist for transforming an image from spatial space to frequency space, including the Discrete Cosine Transform (DCT)~\cite{ahmed1974discrete}, Discrete Fourier Transform (DFT)~\cite{winograd1978computing}, and Wavelet Packet Decomposition (WPD)~\cite{xiong1998wavelet}. 
% Among these methods, WPD provides a unique multi-scale frequency domain analysis, effectively capturing features of images at various scales. This analysis not only enhances our overall understanding of the image's structural compositions but also makes WPD particularly adept at precisely locating and representing local image features with distinct semantic meanings within the frequency domain. Consequently, WPD facilitates a more detailed analysis of frequency information distribution within the dataset, enabling us to select key frequency regions in the spectrogram for trigger injection to achieve successful backdoor attacks at low poisoning ratios.
% Among these methods, WPD can provide a unique multi-scale frequency domain analysis. This allows WPD to effectively capture features at various image scales, thereby enhancing the overall understanding of the image's structural composition. Furthermore, WPD excels in accurately locating and representing local image features with different semantic meanings within the frequency domain.
% Specifically, we leverage the capability of the wavelet packet decomposition (WPD)~\cite{xiong1998wavelet}, which decomposes one image to different frequency regions, such that we can obtain frequency information with different semantic meanings. 
% Utilizing WPD, we selectively modify the key frequency regions in the spectrogram based on the frequency information distribution within the dataset.
% With the aim of proposing a precise and stable attack method, we leverage the capability of WPD to selectively modify the key frequency regions in the spectrogram based on the distribution of frequency information in the dataset. 
Furthermore, we also conduct qualitative analyses to improve the trigger to promote the model to learn the trigger information more effectively. Additionally, we offer visualization analyses based on $l_2$-distance Kernel Density Estimation (KDE) to explain the reasons for the effectiveness of our method at low poisoning ratios.
% we explain why our method works at low poisoning ratios.
% And we also leverage the generalization of the model to set the same mode with different parameters to generate the poisoned training samples and the poisoned test samples, which can balance the attack performance and the naturalness of poisoned samples.
% improve the naturalness of the poisoned testing samples.\\
% \\
% \hspace*{0.15cm}

The main contributions of this work includes the following four aspects:
\begin{itemize}
\item We leverage WPD to analyze the frequency information distribution within datasets. This analysis helps us infer the regions of information that models are likely to focus on, leading to the development of dataset-specific poisoning strategies for enhanced attack effectiveness. 
% Considering the inherent information biases present across diverse datasets, we leverage WPD to analyze their frequency distributions. This analysis enables us to infer key frequency regions likely to attract the attention of DNNs, leading to the development of dataset-specific poisoning strategies for enhanced attack effectiveness.
% We explore the frequency distribution of different datasets by WPD to infer which frequency regions the NNs would focus on.
\item We develop an attack method based on data poisoning, referred to as WPDA, which is characterized by its efficiency, stealth, and stability. This method can achieve a high ASR even at low poisoning ratios, and it is capable of evading most existing defense methods.
% We propose a data-poisoning based attack method, denoted as WPDA, which can achieve a desired ASR even at extremely low poisoning ratios.
% \item We conduct qualitative analyses to explore the effect of the backdoor's characteristics on the model in order to improve the effectiveness of the attack methods.
\item Comprehensive experimental evaluations show the superior results of our method, especially at the low poisoning ratios. Besides, extensive qualitative analyses reveal the reasons for the effectiveness of WPDA.
\item We provide $l_2$-distance Kernel Density Estimation (KDE) visualization analyses to explain underlying mechanism and demonstrate that our method promotes the model effectively learn the trigger rather than memorizing the poisoned training samples.
\end{itemize}
\textbf{Organization.}
The structure of the remainder of the paper is outlined as follows: 
% In the next section, we list related work on backdoor attacks, backdoor defense.
% In the next section
In Section~\ref{related work}
, we provide a comprehensive review of related work pertaining to backdoor attacks and defenses.
Following this, we introduce the preliminary theory of the wavelet packet transform and define the problem formulation. We describe the implementation of our method in detail in Section~\ref{Method}. In Section~\ref{Experiment}, We compare our method with 7 SOTA attack methods in terms of attack performance and defense performance. In Section~\ref{tsne-kde}, we conduct t-SNE and $l_2$-distance KDE visualization experiments to analyze our method and other attacks. Finally, we conclude our work in Section~\ref{conclusion}.
% We hope that our work can offer some new ideas for the development of the backdoor field.

% Next, we present the preliminary theory of the wavelet packet transform and the problem formulation. Based on the results of the dataset analysis, We initially propose our method and optimize the trigger through qualitative analyses. The implementation is shown in Section ~\ref{Method}. In Section ~\ref{Experiment}, We compare our method with 7 SOTA attack methods in terms of attack performance and defense performance. In addition, we also conduct visualization experiments to analyze our method  and compare it with others. We conclude our work in Section ~\ref{conclusion}. We hope that our work can offer some new ideas for the development of the backdoor field.



==> tip/2_Introduction_new.tex <==
\section{Introduction}
\IEEEPARstart{D}{eep}
neural networks (DNNs) have achieved remarkable success and widespread adoption in various research fields (\eg, face recognition~\cite{balaban2015deep}, voice recognition~\cite{li2012improving,yuan2018commandersong}, and autonomous driving~\cite{zhou2020deepbillboard}), leading to significant advancements in artificial intelligence. However, this progress also introduces potential security vulnerabilities. 
Among these security threats, backdoor attacks pose a significant risk, involving maliciously manipulating a DNN model during training to embed hidden backdoors. These backdoors can be triggered by specific input patterns, causing the model to produce targeted incorrect outputs while maintaining normal performance on benign inputs. The implications of such attacks range from targeted misclassification and data manipulation to compromising the integrity and reliability of critical systems that rely on DNNs.

In this work, we study the threat model of data poisoning- based backdoor attack, where the attack can only manipulate the training dataset, without access to the training process. It applies to the practical scenario that the user doesn't have sufficient training data, thus download or buy data from an untrustworthy third-party data platform. Although several effective backdoor attacks have been developed, they often require a substantial number of poisoned training samples to achieve the desired attack success rate, potentially increasing the risk of being detected by detection methods or defended by defense methods. Our goal is to achieve a precious attack at low poisoning ratios, which is necessary and challenging~\cite{wu2022backdoorbench}. 
In scenarios of backdoor attacks with a low poisoning ratio, the primary challenge is ensuring that the model can effectively learn the trigger from a limited number of poisoned training samples. 
\textit{The key to overcoming this challenge lies in inferring the important regions of datasets information that the models focus on during the training process and strategically injecting the trigger into these regions. 
}
Several studies~\cite{wang2020high,ilyas2019adversarial,rahaman2019spectral,abello2021dissecting,wang2023neural}
demonstrate that DNNs can learn the frequency information of images and benefit from specific frequency information. Therefore, we focus on identifying key regions in the frequency domain.
Currently, several techniques exist for transforming an image from spatial space to frequency space, including the Discrete Cosine Transform (DCT)~\cite{ahmed1974discrete}, Discrete Fourier Transform (DFT)~\cite{winograd1978computing}, and Wavelet Packet Decomposition (WPD)~\cite{xiong1998wavelet}. 
Among these methods, WPD provides a unique multi-scale frequency domain analysis, effectively capturing features of images at various scales. This analysis not only enhances our overall understanding of the image's structural compositions but also makes WPD particularly adept at precisely locating and representing local image features with distinct semantic meanings within the frequency domain. Consequently, WPD facilitates a more detailed analysis of frequency information distribution within the dataset, enabling us to select key frequency regions in the spectrogram for trigger injection to achieve successful backdoor attacks at low poisoning ratios.

The authors in\cite{wang2023neural,abello2021dissecting} illustrate that important frequency regions that DNNs focus on in classification should be data-driven. Existing works on frequency-domain based backdoor attacks~\cite{drager2022backdoor} adopt a fixed selection strategy in selecting poisoning regions, ignoring the differences between various datasets, which results in suboptimal performance. Hence, instead of following their strategy, we conduct an in-depth analysis of the characteristics of different datasets and propose a dataset-specific strategy for selecting poisoning regions.

The main contributions of this work includes the following aspects:
\begin{itemize}
\item We leverage WPD to analyze the frequency information distribution within datasets. This analysis helps us infer the regions of information that models are likely to focus on, leading to the development of dataset-specific poisoning regions selection strategy for enhanced attack effectiveness. 
\item We develop an attack method based on data poisoning, referred to as WPDA, which is characterized by its effectiveness, stealthiness, and stability. This method can achieve a high ASR even at low poisoning ratios, and it is capable of evading most existing defense methods.
\item Comprehensive experiments and analyses are provided to explain underlying mechanism and demonstrate that our method promotes the model effectively learn the trigger rather than memorizing the poisoned training samples.
\end{itemize}
\textbf{Organization.}
The structure of the remainder of the paper is outlined as follows: 
% In the next section, we list related work on backdoor attacks, backdoor defense.
% In the next section
In Section~\ref{related work}
, we provide a comprehensive review of related work pertaining to backdoor attacks and defenses.
Following this, we introduce the preliminary theory of the wavelet packet transform and define the problem formulation. We describe the implementation of our method in detail in Section~\ref{Method}. In Section~\ref{Experiment}, We compare our method with 7 SOTA attack methods in terms of attack performance and defense performance. In Section~\ref{tsne-kde}, we conduct t-SNE and $l_2$-distance KDE visualization experiments to analyze our method and other attacks. Finally, we conclude our work in Section~\ref{conclusion}.


==> tip/3_relatedwork.tex <==
\section{Related Work}
\label{related work}
\subsection{Backdoor Attack}
Current research about backdoor attacks can be interpreted as the process of maliciously implanting a backdoor into the model, which would induce the model to build the relationship between special input triggers with a desired output. The main methodologies include poisoning training data~\cite{gu2019badnets,chen2017targeted,li2021invisible,shafahi2018poison,gao2023imperceptible}, manipulating the model's parameters~\cite{kurita2020weight
% ,9737144
}, or controlling the training process~\cite{
shumailov2021manipulating, 
nguyen2021wanet,nguyen2020input,bagdasaryan2021blind,jiang2022incremental}. In particular, attackers can manipulate both images and labels~\cite{gu2019badnets,chen2017targeted,li2021invisible} in data poisoning works.

% there are two types of attack settings, in one of which attackers can manipulate both images and labels~\cite{gu2019badnets,chen2017targeted,li2021invisible}, while in the other setting that attackers can only modify labels~\cite{shafahi2018poison,zhao2020clean}. 
BadNets~\cite{gu2019badnets} is a pioneering work on backdoor attacks in image classification tasks that injects a white patch into benign samples. Subsequent research has explored various backdoor attack techniques, including Blended~\cite{chen2017targeted}, which takes a cartoon image as the trigger and blends it with the benign samples. Liu et al.~\cite{liu2020reflection} propose a reflection backdoor attack,  which enhances backdoor attack by applying random spatial transformations to the poisoned image. While such methods have demonstrated effectiveness, the triggers often introduce noticeable visual artifacts, making them susceptible to detection and removal.
To improve the stealthiness of backdoor attacks, some dynamic invisible trigger generation methods have been proposed, including sample-specific invisible triggers generated by the DNN-based image steganography~\cite{li2021invisible,li2020invisible}, autoencoder neural network~\cite{ning2021invisible,zhang2022poison}, random noise optimizations by adversarial perturbation~\cite{wei2022adversarial,zhang2021advdoor,wang2021psat,che2021adversarial}, image warping~\cite{nguyen2021wanet,cheng2020deep} or RGB filter~\cite{gong2023kaleidoscope}, \etc~
\normalsize
Most backdoor attacks mentioned above mainly focus on adding perturbation in the spatial domain. However, Wang et al.~\cite{wang2021backdoor} indicated that small perturbations in the frequency domain could produce perturbations dispersed across the entire image, and they proposed a backdoor attack called {\small{FTROJAN}} which injects triggers in mid- and/or high-frequency components of UV channel by Discrete Cosine Transform (DCT). Besides, Feng et al.~\cite{feng2022fiba} embed a trigger into the amplitude spectrum while maintaining the phase spectrum unchanged by utilizing Discrete Fourier Transform (DFT)~\cite{brigham1988fast}. ~\cite{Hammoud_2022_BMVC} generates a poisoning filter based on a Fourier heatmap to poison part of the training samples.

\normalsize
% However, the frequency resolution is limited due to the window size used in the Fourier transform being fixed. In other words, we cannot obtain more abundant frequency information from input images decomposed. 
% The Fourier Transform treats the image as a whole, which means that it can only compute the spectrum of the whole image
% and cannot provide local frequency information
% . In contrast, the wavelet transform can extract local frequency information.
Unlike DFT and DCT, which focus primarily on global frequency representations, the wavelet transform offers the advantage of capturing both frequency and spatial information. This allows for the extraction of detailed features such as edges, contours, and textures, providing a more comprehensive understanding of image characteristics. Additionally, the multi-resolution analysis capabilities of the wavelet transform enable the decomposition of information at various scales, further enhancing the precision of feature extraction.
% To overcome this drawback, 
Drager et al.~\cite{drager2022backdoor} propose a wavelet transform-based attack (WABA) method which injects the trigger image into the lowest-frequency components of poisoned images by wavelet transform. 
However, in most cases, it is difficult to maintain the naturalness of the poisoned images by injecting trigger information into the low-frequency region.
Wavelet packet decomposition (WPD) is an improvement based on the wavelet transform, which is able to subdivide both high and low frequency information, while wavelet transform can only subdivide low frequency information. 
% Analysis of the dataset by WPD to infer the key frequency regions of attention of the DNNs contributes to the proposal of an effective and accurate backdoor attack method, as well as easy control of the naturalness of the poisoned images.
Analysing the dataset by WPD to infer the key frequency regions that the DNNs focus on is conducive to the proposal of an effective and precise backdoor attack method. In addition, how to design the trigger information to ensure the effectiveness of the backdoor attack while also making the poisoned images stealthy needs to be further explored.


\subsection{Backdoor Defense}
\normalsize
Backdoor defense can be broadly divided into three categories, which are pre-training, in-training, and post-training. For pre-training methods, the defender aims to detect poisoned samples in the training dataset by capturing the anomalous behavior characteristics of poisoned samples, such as activation of samples (\textit{e.g.} AC\cite{chen2018detecting}, Beatrix\cite{mabeatrix}, SCAn\cite{tang2021demon}, Spectral\cite{tran2018spectral}, and SPECTRE\cite{hayase2021spectre}) and the prediction consistency of samples (\textit{e.g.} CT\cite{qitowards} and ASSET\cite{asset}). For in-training methods, defenders distinguish poisoning samples and benign samples by the difference of their training loss \cite{li2021anti} or feature gathering \cite{huang2022backdoor, chen2022effective,zeng2021adversarial}, and then unlearn these samples or securely retrain a clean model on the processed dataset. For post-training methods, the defenders remove the embedded backdoors by snipping out possible backdoor neurons, including CLP~\cite{zheng2022data}, and NAD~\cite{li2021neural}, or fine-tuning the backdoored model to mitigate backdoor~\cite{wei2023shared,zhu2023neural,yao2024reverse}. 
Furthermore, defenders are capable of reversing backdoor triggers and then pruning backdoor models using these trigger-stamped samples, such as in the NC~\cite{wang2019neural} method, or by rejecting queries once the inputs are identified as poisoned samples (\textit{e.g.} STRIP\cite{gao2019strip}
% , SCALE-UP\cite{SCALE-UP}, 
and TeCo\cite{liu2023detecting}).

==> tip/4_method.tex <==
\section{Method}
\label{Method}
\subsection{Preliminary}
Wavelet Packet Decomposition (WPD) can transform an image from the spatial domain to the frequency domain and decompose it into multiple frequency regions containing different semantic information. It
inherits the time-frequency analysis characteristics of the wavelet decomposition (WD). The main difference is that WD can only decompose low frequency, while WPD can decompose information in every frequency band. The input image $x$ is transformed to a spectrogram which contains low frequency `a', high-horizontal frequency `h', high-vertical frequency `v', high-diagonal frequency `d'. Taken an image from CIFAR-10 as an example in the Fig.~\ref{WPD}, the image in the level-2 spectrogram contains 16 sub-spectrograms with different semantic information.
% Fig.~\ref{WPD} briefly illustrates the process of level-N WPD.
\begin{figure}[htbp]
\centering
\includegraphics[width=3in]{figures/WPD.pdf}
\caption{The principle of wavelet packet decomposition.}
\label{WPD}
\end{figure}
\vspace{-0.5cm}
\subsection{Problem Formulation}
\paragraph{\textbf{Notations}}
\normalsize
We denote a deep learning based image classifier as $f_{\btheta}: \mathcal{X} \rightarrow \mathcal{Y}$, where $\btheta$ is the model parameter, $\X \in \mathbb{R}^3, \Y = \{1, 2, \ldots, c\}$ indicate the input and output space, respectively. The benign training dataset is denoted as $\D = \{(\x^{(i)}, y^{(i)})\}_{i=1}^n$, where $\x^{(i)} \in \X$ denotes a benign image, while $y^{(i)}$ is its ground-truth label. It will be splitted to two parts, including $\D_c$ and $\D_p$, and the images in $\D_p$ are selected to generate poisoned images, \ie, $(\x^{(i)}, y^{(i)})$ is modified to $(\x_{\triangle}^{(i)}, t)$ by injecting a trigger \textit{$\triangle$} into $\x^{(i)}$ and changing $y^{(i)}$ to the target label $t$. The set of poisoned image pairs is denoted as $\hat{\D}_p = \{(\x_{\triangle}^{(i)}, t) | (\x^{(i)}, y^{(i)}) \in \D_p \})$. 
Then, the poisoned training dataset is $\hat{\D} = \{\D_c, \hat{\D}_p\}$, 
and the poisoning ratio is $p = \frac{|\hat{\D}_p|}{|\hat{\D}|}$.
\paragraph{\textbf{Threat Model}}
\vspace{0.2cm}
\normalsize
In this work, we consider the data-poisoning based backdoor attack, where the attacker can only manipulate the benign training dataset $\D$ to obtain the poisoned training dataset $\hat{\D}$, without access to the training process.
At the inference stage, given the model $f_{\btheta}$ trained on $\hat{\D}$ by the user, the attacker can generate the poisoned image  by injecting the  trigger pattern into the benign inference image, and aims to activate the backdoor in the model $f_{\btheta}$, \ie, $f_{\btheta}(\x_{\triangle}) = t$. 

\begin{figure}[htbp]
\centering
\subfigure[Image]{
\includegraphics[width=0.1\textwidth]{figures/img.png}
\label{img}
}
\hspace{0.8cm}
\subfigure[\hspace{-0.05cm}Image without low frequency]{
\label{img_without_low}
\includegraphics[width=0.1\textwidth]{figures/img_without_low.png}
}
\hspace{0.8cm}
\subfigure[Image without high frequency]{
\label{img_without_high}
\includegraphics[width=0.1\textwidth]{figures/img_without_high.png}
}
\caption{The influence of high and low frequency information on image vision.}
\label{The influence of high and low frequency information on image vision}
\end{figure}
\vspace{-0.5cm}
\subsection{Analysis on Dataset}
\label{Analysis on dataset}
In order to make the attack methods more stealthy and precise, we analyze the datasets to infer the key frequency regions within the spectrograms that DNNs would focus on. These key frequency regions will then be selected as the poisoning regions for our attack. By employing N-level WPD, we decompose the frequency information of training samples in the datasets, resulting in $4^N$ sub-spectrograms within $4^{N-1}$ parent-spectrograms, where each parent-spectrogram encompasses 4 sub-spectrograms. To quantify the information content and importance of each sub-spectrogram, we calculate the effectiveness $E$ of the frequency information within each sub-spectrogram across all training samples in dataset $\D$. As defined in Eq. \eqref{effectiveness of the frequency information}, $E$ represents the magnitude of the absolute average of the coefficient matrix within each sub-spectrogram. This approach helps to mitigate the influence of noise and highlight the regions containing the most prominent and relevant information.
% \begin{equation}
% \label{effectiveness of the frequency information}
% E^N_{s,p} = \sum_{x^{(i)}\in \D}^{} {\left |avg(C^N_{s,p})  \right |},
% \end{equation}
% \vspace{-0.5cm}
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{3pt}
\begin{equation}
\label{effectiveness of the frequency information}
\left\{
             \begin{array}{lr}
             {C^N_{s,p}} = \{\sum\limits_{x^{(i)}\in \D}^{}{\mathcal{W}^{N}(x^{(i)})\}_{s,p}}, &
             \vspace{0.2cm}\\
             E^N_{s,p} = {\left | \text{avg}(C^N_{s,p})  \right |},&  
             \end{array}
\right.
\end{equation}}
\\
where $C^N_{s,p} $ represents the coefficient matrix of s-th sub-spectrogram in p-th parent-spectrogram, and $s \in [1,4]$, $p \in [1,4^{N-1}]$. $\mathcal W$ represents WPD, which converts the image from the spatial domain to the spectrogram, $N$ is the level of WPD. Considering that the images in the training dataset might be affected by various factors during the acquisition process, such as sensor limitations, transmission errors, or environmental factors, which might introduce noise. Noise usually has a lower amplitude, and its contribution to the absolute average value is relatively minor compared to that of the actual signal. (The relevant proof will be shown in Appendix ~\ref{appendix}.) This implies that sub-spectrograms with higher $E$ values are more likely to contain significant information or features of interest, rather than being predominantly composed of noise. This understanding is crucial for effectively analyzing and extracting reliable features from the dataset.
As a result, we refer to the sub-spectrogram with the largest $E$ value in each parent-spectrogram as the key frequency region.
% A larger $E$ indicates the dataset has a higher presence of components within the corresponding sub-spectrogram, and we refer such sub-spectrogram as the key frequency regions. 
We erase the low frequency and high frequency information of an image respectively, and Fig.~\ref{The influence of high and low frequency information on image vision} shows that the lowest frequency information always 
% contains the most information and
plays an impact on image in visual. It is difficult to maintain the visual naturalness after modifying the lowest frequency. Therefore, we do not take into account the information of the lowest frequency when we conduct statistical analysis. 
% \begin{remark}
% $E^N_{s,p}$ is represented as ${\left | \text{avg}(C^N_{s,p})  \right |}$ instead of ${ \text{avg}(\left |C^N_{s,p}\right |)}$. Specially, the elements in $C^N_{s,p}$ include positive and negative values. 
% %Specially, the elements in $C^N_{s,p}$ include positive and negative values. Positive values indicate that the image signal energy is gathered in the direction consistent with the wavelet basis function, and negative values indicate that the image signal energy is gathered in the reverse direction. Considering the direction, we average the coefficient matrix before taking the absolute.
% \end{remark}
% \vspace{-1.5cm}

The complexity of the dataset is affected by the number of categories, image volume, \etc~ The datasets with more categories or larger image volume tend to be more complex and are required to be analysed with more detailed decomposition, \textit{i.e.}, a higher level WPD.
We regard the sub-spectrograms in each parent-spectrogram with most effective information as the key frequency regions. Take CIFAR-10 as an example, Fig.~\ref{CIFAR-10-distribution} illustrates the frequency information distribution of CIFAR-10 decomposed by 2-level WPD, and the parent-spectrograms are the frequency regions in the 1-level WPD, \textit{i.e.}, \textit{`a'}, \textit{`h'}, \textit{`v'}, \textit{`d'}. The lowest frequency \textit{`aa'} is not counted in the statistics. As a result, the sub-spectrograms of \textit{`ah'}, \textit{`ha'}, \textit{`va'}, \textit{`dh'} in each parent-spectrograms contain the most effective information. The details are shown in Algorithm~\ref{alg1}.
\input{tables/algorithm}
\begin{figure}[htp]
\centering
\includegraphics[width=8cm,height =2.2cm]{figures/pie.pdf}
% figures/z_bar.pdf
\caption{Frequency information distribution of CIFAR-10 in \textit{`a'}, \textit{`h'}, \textit{`v'}, \textit{`d'} parent-spectrogram, respectively.}
\label{CIFAR-10-distribution}
\end{figure}
\begin{figure*}[!ht]
\centering
\includegraphics[width=17cm,height =6.3cm]{figures/overview4.pdf}
\caption{Overview of WPDA. 
% The process of data-poisoning backdoor attacks includes three stages. In stage one, attackers design and inject the trigger into the benign samples. In stage two, the poisoned training samples will bootstrap the model to change decision boundaries during training process. In stage three, the model trained by poisoned training samples can classify the poisoned testing samples into the target class and the benign testing samples into the original class.
\textit{Poisoned Samples Generation} module describes the process of poisoned samples generation, including the poisoned training and the poisoned testing samples.
}
\label{overview}
\end{figure*}
\vspace{-0.7cm}
\subsection{Proposed Method}
\label{method}
Here we elaborate the proposed WPD-based backdoor attack, dubbed \textbf{WPDA}. Since we focus on data-poisoning based attack, we only describe how to generate the poisoned dataset and inject backdoor, including three main steps in Fig.~\ref{overview}:
\begin{enumerate}[]
\item Generating the poisoned training samples. Following Algorithm~\ref{alg1}, we select $4^{N-1}$ key frequency regions identified as the most informative portions of the parent-spectrograms. These regions are designated as poisoning frequency regions for the attack. The generation of poisoned training samples, denoted as $\hat{\boldsymbol{x}}_{train}$, is then performed according to Eq. \eqref{poisoned_training_samples_generation_equation}: 
% Selecting $4^{N-1}$ key frequency regions as the poisoning frequency regions according to Algorithm~\ref{alg1} and generating the poisoned training samples $\hat{\boldsymbol{x}}_{train}$ by Eq. \eqref{poisoned_training_samples_generation_equation}: 
\begin{equation}
% \footnotesize
\begin{aligned}
\label{poisoned_training_samples_generation_equation}
g({x}_{train};k) = \mathcal W^{-N}(\mathcal W&
^N (x_{train})\odot m + k \cdot (\mathcal T(\mathcal W^N(\triangle)) &  \\
\odot (1-m))),
% \g({x}_{train};k) &=\mathcal W^{-1} ((k \cdot (\mathcal T(\mathcal W(\xi))) + \alpha  \cdot 
% \mathcal W (x_{train}))\odot (1-m) \\& + \mathcal W (x_{train})\odot m) ,
\end{aligned}
\end{equation}
% \hspace*{0.65cm}
where $\hat{\boldsymbol{x}}_{train} = g({x}_{train};k)$, $\triangle$ represents the trigger image, $m \in \left \{ 0,1 \right \} ^{2^N\times2^N\times 3}$ is a binary mask, $k$ is the trigger intensity of the poisoned training samples $\hat{\boldsymbol{x}}_{train}$.
% According to \ref{simplicity of trigger information}, 
% To make the trigger image unrestricted and enhance its visual convert, 
To further enhance the stealthiness and effectiveness of the attack, we apply averaging-transformation $\mathcal{T}$ to the trigger within the spectrogram. This averaging-transformation involves replacing each element value with the average value of the coefficients within the corresponding sub-spectrogram. Through the averaging-transformation,  we achieve two key objectives: (1) simplifying the trigger information while preserving its essential characteristics, and (2) reducing visual artifacts that might raise suspicion during visual inspection of the poisoned samples.
% We perform a transformation $\mathcal{T}$ of the trigger in the spectrogram, \textit{i.e.}, each element value is replaced by the average value of the coefficient in sub-spectrogram. The transformation $\mathcal{T}$ not only simplifies the trigger information but also improves the stealthiness of the trigger in visual. 
In the poisoned training samples, we mask information of the original image in the poisoning frequency regions to promote the model to effectively capture and learn the trigger information.  
\item Backdoor injection. 
Backdoor are injected into the model when the user trains the model by the poisoned training dataset $\hat{\mathcal D_p}$. The loss function for model training is shown in Eq. \eqref{attack_equation}:
\begin{equation}
\label{attack_equation}
% \min \limits_{\theta} \mathcal L (f_{\theta }(x_{train};\text{k}), t),
\min \limits_{\theta} \mathcal L ((f_{\theta }({\hat{\boldsymbol{x}}_{train}}), t) + (f_{\theta }( {x}_{train}), y)
).
\end{equation}
\item Generating the poisoned testing samples.
In practical application scenarios, we need to consider the visual performance of the poisoned testing samples, so we retain the information of the original image with the intensity of $\alpha$ in the poisoning frequency regions at the stage of generating the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$.
The poisoned testing samples are generated as Eq. \eqref{poisoned_test_samples_generation_equation}:
\begin{equation}
% \footnotesize
\label{poisoned_test_samples_generation_equation}
\begin{aligned}
{g \prime}({x}_{test};{k^ \prime}
) 
&=\mathcal W^{-N} (({k^ \prime}  \cdot (\mathcal T(\mathcal W^N(\triangle))) + \alpha  \cdot \mathcal {W}^N (x_{test})) \\& 
\odot (1-m) +
 \mathcal {W}^N (x_{test})\odot m) ,
\end{aligned}
\end{equation}
where $\hat{\boldsymbol{x}}_{test} = g({x}_{test};k')$, $k'$ is the trigger intensity and $\alpha$ is the original sample information intensity of the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$.
\end{enumerate}
\vspace{-0.3cm}
\subsection{Qualitative Analyses}
\label{Qualitative Analysis}
In the deployment of backdoor attacks, the three core elements of trigger design are the \textbf{stealthiness}, \textbf{efficiency} and \textbf{stability}. Stealthiness ensures that backdoor samples are not easily detected by the human eye during deployment; efficiency ensures that the backdoor can rapidly and precisely execute malicious operations upon activation; stability ensures that the backdoor works reliably under various conditions and environments, even when interfered by diverse factors.\\
\noindent
\textbf{How to generate stealthy triggers $\rightarrow \mathcal T$.} We use the averaging-transformation $\mathcal T$ on the trigger to improve the stealthiness of the trigger. Fig.~\ref{stealthy} illustrates original sample and backdoor samples with averaging-transformation or not. Based on mean square error(MSE) and structural similarity index measure(SSIM), we demonstrate that averaging-transformation can effectively improve the stealthiness of the trigger.\\
\begin{figure}[H]
\vspace{-0.5cm}
\centering
\includegraphics[width=8.8cm,height =3.5cm]{figures/stealthy2.pdf}
\caption{The benign samples and the backdoor samples generated without and with averaging-transformation $\mathcal T$. SSIM and MSE values represent the average measurements calculated from training samples in the CIFAR-10. Higher SSIM values and lower MSE values indicate greater similarity between the samples.}
\label{stealthy}
\end{figure}
\vspace{-0.15cm}
\noindent
\textbf{How to generate effective triggers $\rightarrow k$.} In the training process, the original sample information compete with the trigger information for the model's attention, making it harder for the model to learn the association between the trigger and the target label. (The relevant proof will be shown in Appendix\ref{original information have negative effect on the backdoor activation}) To address this, we mask the original sample information in the poisoning frequency regions before injecting the trigger. Besides, we use the hyperparameter $k$ to adjust the intensity of the trigger information. We expect the information of the trigger to be more prominent than that of the original image, so we explore the effect of the value of $k$ on the backdoor activation. Fig.~\ref{prominence} illustrates the value of $k$ has a significant impact on the backdoor activation at low poisoning ratios, and backdoor activation at low poisoning ratios require a large value of $k$. As a result, We select the largest $k$ value as permitted by the stealthiness of the trigger.\\
\begin{figure}[H]
\vspace{-0.7cm}
\centering
\includegraphics[width=6.4cm,height =3.9cm]{figures/zcifar10_intensity_11.pdf}
\caption{We evaluate the effect of the value of $k$ on backdoor activation on  PreAct-ResNet18 and VGG19-BN trained by CIFAR-10 with different poisoning ratios, and use poisoned vaildation set to test the accuracy of backdoor activation.}
\label{prominence}
\end{figure}
\noindent\textbf{How to generate stable trigger $\rightarrow \alpha$ and $k'$.} To ensure the stability of the trigger, we need to balance the generalization of the model and the naturalness of the backdoor samples. Regarding this, we design the hyperparameters $\alpha$ and $k'$ during the process of generating poisoned testing samples. We explore the generalization of the model trained with different poisoning ratios on the original image information and the trigger information, respectively. Fig.\ref{The generalization of the model on the original image information} illustrates that the model perceives the original image information as noise-like, and the larger the original sample information intensity $k'$ is, the more difficult it is for the backdoor to be activated. Besides, we observe that the lower the poisoning ratio is, the more limited the generalization of the model is. Fig.\ref{The generalization of the model on the trigger information} illustrates that the model trained with low poisoning ratios are is less sensitive to trigger information than that with high poisoning ratios. In other words, the backdoor activation requires large trigger information intensity $k'$, especially for the model trained with low poisoning ratios. As a result, we can flexibly set the values of $\alpha$ and $k'$ when generating poisoned testing samples based on the poisoning ratios.

\begin{figure}[htbp]
\vspace{-2.8mm}
\centering
\subfigure[The generalization of the model on the original image information]{
% \includegraphics[width=0.20\textwidth]
\includegraphics[width=3.8cm,height=3.1cm]
{figures/zCIFAR10_generation_orir_v1_111.pdf}
\label{The generalization of the model on the original image information}
}
\hspace{3mm}
\subfigure[The generalization of the model on the trigger information]{
% \includegraphics[width=0.22\textwidth]
\includegraphics[width=3.5cm,height=3.1cm]
{figures/zCIFAR10_generation_trigger_v1_111.pdf}
\label{The generalization of the model on the trigger information}
}
\caption{We evaluate the generalization of the model trained with different
poisoning ratios to the original samples information and trigger information, respectively. Taking VGG9-BN trained by CIFAR-10 as an example. (a) Fixed the trigger information intensity $k'=6$ in the poisoned vaildation samples, we use the poisoned vaildation set to test the accuracy of backdoor activation and adjust the original sample information intensity $\alpha$ in the poisoned vaildation samples to test the accuracy of backdoor activation. (b) Fixed the original sample information intensity $\alpha=1$ in the poisoned vaildation samples, we use the poisoned vaildation set to test the accuracy of backdoor activation and adjust the trigger information intensity $k'$ in the poisoned vaildation samples to test the accuracy of backdoor activation.
% confirm the generalization of the model on the trigger information.
% Taking CIFAR-10 trained on VGG19-BN as an example. In the \textbf{left}, we set $k=6$ and analyze the effect of the intensity of the original image information $\alpha$ on the generalization of the model. In \textbf{right}, we set $\alpha = 1$ and analyze the effect of the intensity of the trigger information $k'$ on the generalization of the model.
}
\label{fig:generation}
\end{figure}

% \begin{figure}[H]
%   \begin{minipage}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[scale=0.17]
% \includegraphics[width=4.2cm,height=2.8cm]{figures/zcifar10_consistency_11.pdf}
%     \caption{Simplicity of trigger.}
%     \label{simplicity}
%   \end{minipage}%
%   \begin{minipage}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[scale=0.143]
% \includegraphics[width=4.2cm,height=2.8cm]{figures/zcifar10_intensity_11.pdf}
%     \caption{Impact of varying values of $k$ on backdoor activation under different poisoning ratios.}
%     \label{prominence}
%   \end{minipage}
% \end{figure}
% \paragraph{\textbf{Simplicity}} 
% \label{simplicity of trigger information}
% Take CIFAR-10 as an example and we choose ``Hello Kitty'' image as the source to generate trigger information. The improvement of the trigger is approached from three perspectives: simplicity, prominence and stealth. \textit{Simplicity} describes the simplicity of the frequency domain information of the trigger; \textit{Prominence} describes the prominence of the trigger message to the model; \textit{Stealthiness} describes the visual invisibility of triggers in the poisoned samples. 
% We generate a validation dataset using the same model as the poisoned training dataset and analyse the impact of triggers with different characteristics on the model based on the accuracy of the model on the validation dataset.
% % \begin{figure}[H]
% %   \begin{minipage}[t]{0.5\linewidth}
% %     \centering
% %     % \includegraphics[scale=0.17]
% % \includegraphics[width=4.2cm,height=2.8cm]{figures/zcifar10_consistency_11.pdf}
% %     \caption{Simplicity of trigger.}
% %     \label{simplicity}
% %   \end{minipage}%
% %   \begin{minipage}[t]{0.5\linewidth}
% %     \centering
% %     % \includegraphics[scale=0.143]
% % \includegraphics[width=4.2cm,height=2.8cm]{figures/zcifar10_intensity_11.pdf}
% %     \caption{Impact of varying values of $k$ on backdoor activation.}
% %     \label{prominence}
% %   \end{minipage}
% % \end{figure}
% % \paragraph{\textbf{Simplicity}} 
% % \label{simplicity of trigger information}
% We change the simplicity of the trigger information by adding Gaussian noise to the trigger, and Gaussian noise with large varience will decrease the simplicity of the trigger among the poisoned samples. We train the model using training samples with Gaussian noise and then test the performance of the model using validation samples with Gaussian noise. Fig.~\ref{simplicity} illustrates that complex triggers increase the difficulty for models to learn triggers.
% The models with high poisoning ratios are better at learning triggers than the model with low poisoning ratios,
% % The model with low poisoning ratios are less stable than the model with high poisoning ratios, 
% which means simple trigger information is more conducive to the effective attack of models with low poisoning ratios.

% \paragraph{\textbf{Prominence}}
% \label{prominence of trigger information}
% In order to guide the model to focus on the trigger information, we erase the original information in the poisoning frequency regions and then add the trigger with different intensty $k$. We control the prominence of trigger information by modifying the $k$ value, then analyze the effects of triggers with different $k$ value on the model according to accuracy of the poisoned validation dataset. Fig.~\ref{prominence} illustrates that high-intensity trigger information can improve the effectiveness of the attack on both PreAct-ResNet18 and VGG19-BN, especially at extremely low poisoning ratios. 
% % \begin{figure}[htbp]
% % \vspace{-2.8mm}
% % \centering
% % \subfigure[The generalization of the model on the original image information]{
% % % \includegraphics[width=0.20\textwidth]
% % \includegraphics[width=3.8cm,height=3.1cm]
% % {figures/zCIFAR10_generation_orir_v1_111.pdf}
% % \label{The generalization of the model on the original image information}
% % }
% % \hspace{3mm}
% % \subfigure[The generalization of the model on the trigger information]{
% % % \includegraphics[width=0.22\textwidth]
% % \includegraphics[width=3.5cm,height=3.1cm]
% % {figures/zCIFAR10_generation_trigger_v1_111.pdf}
% % \label{The generalization of the model on the trigger information}
% % }
% % \caption{Taking CIFAR-10 trained on VGG19-BN as an example. In the \textbf{left}, we set $k=6$ and analyze the effect of the intensity of the original image information $\alpha$ on the generalization of the model. In \textbf{right}, we set $\alpha = 1$ and analyze the effect of the intensity of the trigger information $k'$ on the generalization of the model.}
% % \label{fig:generation}
% % \end{figure}
% % \vspace{-1mm}
% \paragraph{\textbf{Stealthiness}} 
% \label{stealthiness of trigger information}
% We suppose that the original information has the negative effect on the backdoor activation, but the model has a limited generalization ability. After assuring that the model is able to learn the trigger information effectively (\textit{i.e.}, the triggers are prominent enough and the trigger information is simple enough during the training stage), we retain the frequency information of the original image with the intensity $\alpha$ to the poisoned validation samples and analyze the generalization of the models under different poisoning ratios according to the accuracy of the poisoned validation dataset. There are obvious differences in the generalization of models with different poisoning ratios in Fig.~\ref{The generalization of the model on the original image information}. When $\alpha$ increases, the accuracy of the poisoned validation dataset gradually decreases. While, the backdoor models trained by the datasets with high concentration of poisoned samples have strong  generalization ability.
% Similarly, we set $\alpha = 1$ and modify the trigger intensity $k'$ in the poisoned validation dataset. As shown in Fig.~\ref{The generalization of the model on the trigger information}, poisoned validation samples with intense triggers promote the model to capture the information of the triggers.
% Besides, we also find out that the backdoor models trained by datasets with high concentration of poisoned training samples still have strong generalization ability, which means that their performance reaches over-saturation.
% Therefore, we are supposed to retain the original information with intensity $\alpha$ and set different trigger information intensity $k'$ of the trigger in the poisoned testing samples at different the poisoning ratios.


==> tip/4_method_new.tex <==
\section{Method}
\label{Method}
\subsection{Preliminary}
% Wavelet Packet Decomposition (WPD) can transform an image from the spatial domain to the frequency domain and decompose it into multiple frequency regions containing different semantic information. It
% inherits the time-frequency analysis characteristics of the wavelet decomposition (WD). The main difference is that WD can only decompose low frequency, while WPD can decompose information in every frequency band. The input image $x$ is transformed to a spectrogram which contains low frequency \textit{`a'}, high-horizontal frequency \textit{`h'}, high-vertical frequency \textit{`v'}, high-diagonal frequency \textit{`d'}. Taken an image from CIFAR-10 as an example in the Fig.~\ref{WPD}, the image in the level-2 spectrogram contains 16 sub-spectrograms with different semantic information.
Wavelet Packet Decomposition (WPD) can transform an image from the spatial domain to the frequency domain and decompose it into multiple frequency regions containing different semantic information. It
inherits the time-frequency analysis characteristics of the wavelet decomposition (WD). The main difference is that WD can only decompose low frequency, while WPD can decompose information in every frequency band. Fig.~\ref{WPD} illustrates the process of WPD, transforming an image into spectrogram which contains low frequency \textit{`a'}, high-horizontal frequency \textit{`h'}, high-vertical frequency \textit{`v'}, high-diagonal frequency \textit{`d'}. A further decomposition, such as a 2-level decomposition, results in 16 sub-spectrograms with different semantic information.
% The input image $x$ is transformed to a spectrogram which contains low frequency \textit{`a'}, high-horizontal frequency \textit{`h'}, high-vertical frequency \textit{`v'}, high-diagonal frequency \textit{`d'}. Taken an image from CIFAR-10 as an example in the Fig.~\ref{WPD}, the image in the level-2 spectrogram contains 16 sub-spectrograms with different semantic information.
\begin{figure}[htbp]
\centering
\includegraphics[width=3in]{figures/WPD1.pdf}
\caption{The principle of wavelet packet decomposition.}
\label{WPD}
\end{figure}
\vspace{-0.5cm}
\subsection{Problem Formulation}
\paragraph{\textbf{Notations}}
\normalsize
We denote a deep learning based image classifier as $f_{\btheta}: \mathcal{X} \rightarrow \mathcal{Y}$, where $\btheta$ is the model parameter, $\X \in \mathbb{R}^3, \Y = \{1, 2, \ldots, c\}$ indicate the input and output space, respectively. The benign training dataset is denoted as $\D = \{(\x^{(i)}, y^{(i)})\}_{i=1}^n$, where $\x^{(i)} \in \X$ denotes a benign image, while $y^{(i)}$ is its ground-truth label. It will be splitted to two parts, including $\D_c$ and $\D_p$, and the images in $\D_p$ are selected to generate poisoned images, \ie, $(\x^{(i)}, y^{(i)})$ is modified to $(\x_{\triangle}^{(i)}, t)$ by injecting a trigger \textit{$\triangle$} into $\x^{(i)}$ and changing $y^{(i)}$ to the target label $t$. The set of poisoned image pairs is denoted as $\hat{\D}_p = \{(\x_{\triangle}^{(i)}, t) | (\x^{(i)}, y^{(i)}) \in \D_p \})$. 
Then, the poisoned training dataset is $\hat{\D} = \{\D_c, \hat{\D}_p\}$, 
and the poisoning ratio is $p = \frac{|\hat{\D}_p|}{|\hat{\D}|}$.
\paragraph{\textbf{Threat Model}}
\vspace{0.2cm}
\normalsize
In this work, we consider the data-poisoning based backdoor attack, where the attacker can only manipulate the benign training dataset $\D$ to obtain the poisoned training dataset $\hat{\D}$, without access to the training process.
At the inference stage, given the model $f_{\btheta}$ trained on $\hat{\D}$ by the user, the attacker can generate the poisoned image  by injecting the  trigger pattern into the benign inference image, and aims to activate the backdoor in the model $f_{\btheta}$, \ie, $f_{\btheta}(\x_{\triangle}) = t$. 

\begin{figure}[htbp]
\centering
\subfigure[Image]{
\includegraphics[width=0.1\textwidth]{figures/img.png}
\label{img}
}
\hspace{0.8cm}
\subfigure[\hspace{-0.05cm}Image without low frequency]{
\label{img_without_low}
\includegraphics[width=0.1\textwidth]{figures/img_without_low.png}
}
\hspace{0.8cm}
\subfigure[Image without high frequency]{
\label{img_without_high}
\includegraphics[width=0.1\textwidth]{figures/img_without_high.png}
}
\caption{Effect of high and low frequency information on image vision.}
\label{The influence of high and low frequency information on image vision}
\end{figure}
\vspace{-0.5cm}
\subsection{Analysis on Dataset}
\label{Analysis on dataset}
In order to make the attack methods more stealthy and precise, we analyze the datasets to infer the key frequency regions within the spectrograms that DNNs would focus on. These key frequency regions will then be selected as the poisoning regions for our attack. By employing N-level WPD, we decompose the frequency information of training samples in the datasets, resulting in $4^N$ sub-spectrograms within $4^{N-1}$ parent-spectrograms, where each parent-spectrogram encompasses 4 sub-spectrograms. To quantify the information content and importance of each sub-spectrogram, we calculate the effectiveness $E$ of the frequency information within each sub-spectrogram across all training samples in dataset $\D$. As defined in Eq.~\eqref{effectiveness of the frequency information}, $E$ represents the absolute average magnitude of the absolute average of the coefficient matrix within each sub-spectrogram. This approach helps to mitigate the influence of noise and highlight the regions containing the most prominent and relevant information.
% \begin{equation}
% \label{effectiveness of the frequency information}
% E^N_{s,p} = \sum_{x^{(i)}\in \D}^{} {\left |avg(C^N_{s,p})  \right |},
% \end{equation}
% \vspace{-0.5cm}
% {\setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{3pt}
% \begin{equation}
% \label{effectiveness of the frequency information}
% \left\{
%              \begin{array}{lr}
%              {C^N_{s,p}} = \{\sum\limits_{x^{(i)}\in \D}^{}{\mathcal{W}^{N}(x^{(i)})\}_{s,p}}, &
%              \vspace{0.2cm}\\
%              E^N_{s,p} = {\left | \text{avg}(C^N_{s,p})  \right |},&  
%              \end{array}
% \right.
% \end{equation}}
{\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{3pt}
\begin{align}
    \label{effectiveness of the frequency information}
              E^N_{s,p} &= {\left | \text{avg}(C^N_{s,p})  \right |}, \
              % \label{effectiveness of the frequency information2}
             \textit{where}{\hspace{0.2cm}} {C^N_{s,p}} &= \{\sum\limits_{x^{(i)}\in \D}^{}{\mathcal{W}^{N}(x^{(i)})\}_{s,p}}.   
\end{align}}
% in Eq.~\eqref{effectiveness of the frequency information}, 
\noindent$C^N_{s,p} $ represents the coefficient matrix of s-th sub-spectrogram in p-th parent-spectrogram, and $s \in [1,4]$, $p \in [1,4^{N-1}]$. $\mathcal W$ represents WPD, which converts the image from the spatial domain to the spectrogram, $N$ is the level of WPD. Considering that the images in the training dataset might be affected by various factors during the acquisition process, such as sensor limitations, transmission errors, or environmental factors, which might introduce noise. Noise usually has a lower amplitude, and its contribution to the absolute average value is relatively minor compared to that of the actual signal. (The relevant proof will be shown in Appendix~\ref{explain why it is important to take the average value before taking the absolute value}.) This implies that sub-spectrograms with higher $E$ values are more likely to contain significant information or features of models' interest, rather than being predominantly composed of noise. This understanding is crucial for effectively analyzing and extracting reliable features from the dataset.
As a result, we refer to the sub-spectrogram with the largest $E$ value within each parent-spectrogram as the key frequency region.
% A larger $E$ indicates the dataset has a higher presence of components within the corresponding sub-spectrogram, and we refer such sub-spectrogram as the key frequency regions. 
It should be noticed that when constructing statistical analyses, we do not take into account the information of the lowest frequency. Fig.~\ref{The influence of high and low frequency information on image vision} shows that the lowest frequency information always plays an impact on image in visual, so we refrain from making any alterations to it.

% We remove the low frequency and high frequency information of an image respectively, and Fig.~\ref{The influence of high and low frequency information on image vision} shows that the lowest frequency information always 
% % contains the most information and
% plays an impact on image in visual. It is difficult to maintain the visual naturalness after modifying the lowest frequency. Therefore, we do not take into account the information of the lowest frequency when we conduct statistical analysis. 
% \begin{remark}
% $E^N_{s,p}$ is represented as ${\left | \text{avg}(C^N_{s,p})  \right |}$ instead of ${ \text{avg}(\left |C^N_{s,p}\right |)}$. Specially, the elements in $C^N_{s,p}$ include positive and negative values. 
% %Specially, the elements in $C^N_{s,p}$ include positive and negative values. Positive values indicate that the image signal energy is gathered in the direction consistent with the wavelet basis function, and negative values indicate that the image signal energy is gathered in the reverse direction. Considering the direction, we average the coefficient matrix before taking the absolute.
% \end{remark}
% \vspace{-1.5cm}

The complexity of the dataset is affected by the number of categories, image volume, \etc~ The datasets with more categories or larger image volume tend to be more complex and are required to be analysed with more detailed decomposition, \textit{i.e.}, a higher level WPD.
We regard the sub-spectrograms in each parent-spectrogram with most effective information as the key frequency regions. Take CIFAR-10 as an example, Fig.~\ref{CIFAR-10-distribution} illustrates the frequency information distribution of CIFAR-10 decomposed by 2-level WPD, and the parent-spectrograms are the frequency regions in the 1-level WPD, \textit{i.e.}, \textit{`a'}, \textit{`h'}, \textit{`v'}, \textit{`d'}. The lowest frequency \textit{`aa'} is not counted in the statistics. As a result, the sub-spectrograms of \textit{`ah'}, \textit{`ha'}, \textit{`va'}, \textit{`dh'} in each parent-spectrograms, containing the most effective information, will be selected as poisoning frequency regions. Furthermore, complex datasets require more in-depth decomposition. The details are shown in Algorithm~\ref{alg1}.
\input{tables/algorithm}
\vspace{-0.5cm}
\begin{figure}[htp]
\centering
\includegraphics[width=8cm,height =2.2cm]{figures/pie2.pdf}
% figures/z_bar.pdf
\caption{Frequency information distribution of CIFAR-10 in \textit{`a'}, \textit{`h'}, \textit{`v'}, \textit{`d'} parent-spectrogram, respectively.}
\label{CIFAR-10-distribution}
\end{figure}
% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=17cm,height =6.3cm]{figures/overview10.pdf}
% \caption{Overview of WPDA. 
% \textit{Training Dataset Analysis} module describes the process of analyzing the frequency information distribution of the training dataset using the absolute average algorithm. This analysis identifies the most effective sub-spectrogram within each parent-spectrogram, which are then designated as the poisoning frequency regions. \textit{Backdoor Dataset Generation} module describes the generation process for backdoor samples, which is based on wavelet packet decomposition.
% }
% \label{overview}
% \end{figure*}
\begin{figure*}[!ht]
\centering
\includegraphics
% [width=15cm,height =7.2cm]
[width=14cm,height =6.2cm]
{figures/overview17.pdf}
\caption{Process of WPDA on backdoor samples generation. Before injecting the trigger, we perform frequency distribution statistics on all training samples based on WPD to identify the most informative sub-spectrogram in each parent-spectrogram as the poisoned regions (disregarding the lowest frequency region), and then generate the mask for the backdoor samples generation. In the process of backdoor sample generation, $\mathcal{T}$ represents averaging-transformation.
% \caption{Generation of poisoned training samples for WPDA.
}
\label{overview}
\end{figure*}
\vspace{-0.7cm}
\subsection{Proposed Method}
\label{method}
Here we elaborate the proposed WPD-based backdoor attack, dubbed \textbf{WPDA}. Since we focus on data-poisoning based attack, we only describe how to generate backdoor samples shown in Fig.~\ref{overview}:
\begin{enumerate}[]
% \item  \textbf{Mask Generation}. Following Algorithm~\ref{alg1}, we analyze the frequency distribution of the training dataset based on WPD. $4^{N-1}$ key frequency regions identified as the most informative portions of the parent-spectrograms, and these regions are then designated as poisoning frequency regions for the attack. The information of the poisoning frequency regions in the sa
\item  \textbf{Generating the poisoned training samples}. Following Algorithm~\ref{alg1}, we select $4^{N-1}$ key frequency regions identified as the most informative portions of the parent-spectrograms, and these regions are then designated as poisoning frequency regions for the attack. The generation of poisoned training samples, denoted as $\hat{\boldsymbol{x}}_{train}$, \textit{i.e.}, $g({x}_{train};k)$, is then performed according to Eq.~\eqref{poisoned_training_samples_generation_equation}: 
% Selecting $4^{N-1}$ key frequency regions as the poisoning frequency regions according to Algorithm~\ref{alg1} and generating the poisoned training samples $\hat{\boldsymbol{x}}_{train}$ by Eq. \eqref{poisoned_training_samples_generation_equation}: 
\begin{equation}
% \footnotesize
\begin{aligned}
\label{poisoned_training_samples_generation_equation}
g({x}_{train};k) = \mathcal W^{-N}(\mathcal W&
^N (x_{train})\odot m + k \cdot (\mathcal T(\mathcal W^N(\triangle)) &  \\
\odot (1-m))),
% \g({x}_{train};k) &=\mathcal W^{-1} ((k \cdot (\mathcal T(\mathcal W(\xi))) + \alpha  \cdot 
% \mathcal W (x_{train}))\odot (1-m) \\& + \mathcal W (x_{train})\odot m) ,
\end{aligned}
\end{equation}
% \hspace*{0.65cm}
where 
% $\hat{\boldsymbol{x}}_{train} = g({x}_{train};k)$, 
$\triangle$ represents the trigger image, $k$ is the trigger intensity of the poisoned training samples $\hat{\boldsymbol{x}}_{train}$, $m \in \left \{ 0,1 \right \} ^{2^N\times2^N\times 3}$ is a binary mask.
% According to ~\ref{simplicity of trigger information}, 
% To make the trigger image unrestricted and enhance its visual convert, 
To further enhance the stealthiness and effectiveness of the attack, we apply averaging-transformation $\mathcal{T}$ to the trigger within the spectrogram. This averaging-transformation involves replacing each element value with the average value of the coefficients within the corresponding sub-spectrogram. Through the averaging-transformation, we reduce visual artifacts that can raise suspicion during visual inspection of the poisoned samples, which is verified later in Sec.~\ref{Qualitative Analysis}.
% we achieve two key objectives: (1) simplifying the trigger information while preserving its essential characteristics, and (2) reducing visual artifacts that might raise suspicion during visual inspection of the poisoned samples.
% We perform a transformation $\mathcal{T}$ of the trigger in the spectrogram, \textit{i.e.}, each element value is replaced by the average value of the coefficient in sub-spectrogram. The transformation $\mathcal{T}$ not only simplifies the trigger information but also improves the stealthiness of the trigger in visual. 
In the poisoned training samples, we mask information of the original image in the poisoning frequency regions to promote the model to effectively capture and learn the trigger information.  
% \item \textbf{Backdoor injection}. 
% Backdoor are injected into the model when the user trains the model by the poisoned training dataset $\hat{\mathcal D_p}$. The loss function for model training is shown in Eq.~\eqref{attack_equation}:
% \begin{equation}
% \label{attack_equation}
% % \min \limits_{\theta} \mathcal L (f_{\theta }(x_{train};\text{k}), t),
% \min \limits_{\theta} \mathcal L ((f_{\theta }({\hat{\boldsymbol{x}}_{train}}), t) + (f_{\theta }( {x}_{train}), y)
% ).
% \end{equation}
\item \textbf{Generating the poisoned testing samples}.
In practical application scenarios, we need to consider the visual performance of the poisoned testing samples, so we retain the information of the original image with the intensity of $\alpha$ in the poisoning frequency regions at the stage of generating the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$, \textit{i.e.}, $g'({x}_{test};k')$.
The poisoned testing samples are generated as Eq.~\eqref{poisoned_test_samples_generation_equation}:
\begin{equation}
% \footnotesize
\label{poisoned_test_samples_generation_equation}
\begin{aligned}
{g'}({x}_{test};{k'}
) 
&=\mathcal W^{-N} (({k'}  \cdot (\mathcal T(\mathcal W^N(\triangle))) + \alpha  \cdot \mathcal {W}^N (x_{test})) \\& 
\odot (1-m) +
 \mathcal {W}^N (x_{test})\odot m) ,
\end{aligned}
\end{equation}
where 
% $\hat{\boldsymbol{x}}_{test} = g'({x}_{test};k')$, 
$k'$ is the trigger intensity and $\alpha$ is the original sample information intensity of the poisoned testing samples $\hat{\boldsymbol{x}}_{test}$.
\end{enumerate}
\vspace{-0.3cm}
\subsection{Qualitative Analyses}
\label{Qualitative Analysis}
In the deployment of backdoor attacks, the three core elements of trigger design are the \textbf{stealthiness}, \textbf{effectiveness} and \textbf{stability}. Stealthiness ensures that backdoor samples are not easily detected by the human eye during deployment; effectiveness ensures that the backdoor can rapidly and precisely execute malicious operations upon activation; stability ensures that the backdoor works reliably under various conditions and environments, even when interfered by diverse factors.\\
\noindent
\textbf{How to generate stealthy triggers $\rightarrow \mathcal T$.} We use the averaging-transformation $\mathcal T$ on the trigger to improve the stealthiness of the trigger. Fig.~\ref{stealthy} illustrates original sample and backdoor samples with averaging-transformation or not. Based on mean square error (MSE) and structural similarity index measure (SSIM), we demonstrate that averaging-transformation can effectively improve the stealthiness of the trigger.\\
\begin{figure}[H]
\vspace{-0.7cm}
\centering
% \includegraphics[width=8.8cm,height =3.5cm]
\includegraphics[width=8.0cm,height =3.0cm]
{figures/stealthy5.pdf}
\caption{The benign samples and the backdoor samples generated without and with averaging-transformation $\mathcal T$. SSIM and MSE values are the average measurements calculated from training samples in the CIFAR-10. Higher SSIM values and lower MSE values indicate greater similarity between the samples.}
\label{stealthy}
\end{figure}
\vspace{-0.25cm}
\noindent
\textbf{How to generate effective triggers $\rightarrow k$.} In the training process, the original sample information compete with the trigger information for the model's attention, making it harder for the model to learn the association between the trigger and the target label. (The relevant proof will be shown in Appendix~\ref{original information have negative effect on the backdoor activation}) To address this, we mask the original sample information in the poisoning frequency regions before injecting the trigger. Besides, we use the hyperparameter $k$ to adjust the intensity of the trigger information. We expect the information of the trigger to be more prominent than that of the original image, so we explore the effect of the value of $k$ on the backdoor activation. Fig.~\ref{prominence} illustrates the value of $k$ has a significant impact on the backdoor activation at low poisoning ratios, and backdoor activation at low poisoning ratios require a large value of $k$. As a result, We select the largest $k$ value as permitted by the stealthiness of the trigger.\\
\begin{figure}[H]
\vspace{-0.3cm}
\centering
\includegraphics[width=5.3cm,height =3.1cm]{figures/zcifar10_intensity_111.pdf}
\caption{Effect of the value of $k$ on backdoor activation on  PreAct-ResNet18 and VGG19-BN trained by CIFAR-10 with different poisoning ratios, and use poisoned vaildation set to test the accuracy of backdoor activation.}
\label{prominence}
\end{figure}

\noindent\textbf{How to generate stable triggers $\rightarrow \alpha$ and $k'$.} To ensure the trigger is stably activated, we need to balance the generalization of the model and the naturalness of the backdoor samples. Regarding this, we design the hyperparameters $\alpha$ and $k'$ during the process of generating poisoned testing samples. We explore the generalization of the model trained with different poisoning ratios on the original image information and the trigger information, respectively. Fig.~\ref{The generalization of the model on the original image information} illustrates that the model perceives the original image information as noise-like, and the larger the original sample information intensity $k'$ is, the more difficult it is for the backdoor to be activated. Besides, we observe that the lower the poisoning ratio is, the more limited the generalization of the model is. Fig.~\ref{The generalization of the model on the trigger information} illustrates that the model trained with low poisoning ratios are is less sensitive to trigger information than that with high poisoning ratios. In other words, the backdoor activation requires large trigger information intensity $k'$, especially for the model trained with low poisoning ratios. As a result, we can flexibly set the values of $\alpha$ and $k'$ when generating poisoned testing samples based on the poisoning ratios.

\begin{figure}[htbp]
\vspace{-0.55cm}
\centering
\subfigure[The generalization of the model on the original image information]{
% \includegraphics[width=0.20\textwidth]
\includegraphics[width=3.8cm,height=3.1cm]
{figures/zCIFAR10_generation_orir_v1_111.pdf}
\label{The generalization of the model on the original image information}
}
\hspace{3mm}
\subfigure[The generalization of the model on the trigger information]{
% \includegraphics[width=0.22\textwidth]
\includegraphics[width=3.5cm,height=3.1cm]
{figures/zCIFAR10_generation_trigger_v1_111.pdf}
\label{The generalization of the model on the trigger information}
}
\caption{
% Generalization of the model trained with different poisoning ratios to the original samples information and trigger information, respectively. Taking VGG9-BN trained by CIFAR-10 as an example. (a) Fixed the trigger information intensity $k'=6$ in the poisoned vaildation samples, we use the poisoned vaildation set to test the accuracy of backdoor activation and adjust the original sample information intensity $\alpha$ in the poisoned vaildation samples to test the accuracy of backdoor activation. (b) Fixed the original sample information intensity $\alpha=1$ in the poisoned vaildation samples, we use the poisoned vaildation set to test the accuracy of backdoor activation and adjust the trigger information intensity $k'$ in the poisoned vaildation samples to test the accuracy of backdoor activation.
Generalization of the model trained with different poisoning ratios to the original samples information and trigger information, respectively. Taking VGG19-BN trained by CIFAR-10 as an example, we use the poisoned vaildation set to test the accuracy of backdoor activation, evaluating the model's generalization. (a) Fixed the trigger information intensity $k'=6$ in the poisoned vaildation samples, we adjust the original sample information intensity $\alpha$ in the poisoned vaildation samples to test the accuracy of backdoor activation. (b) Fixed the original sample information intensity $\alpha=1$ in the poisoned vaildation samples, we adjust the trigger information intensity $k'$ in the poisoned vaildation samples to test the accuracy of backdoor activation.
}
\label{fig:generation}
\end{figure}
 

==> tip/5_experiment.tex <==
\section{Experiments}
\label{Experiment}
\subsection{Experiment Settings}
\paragraph{Datasets and Models}
% \noindent\textbf{Datasets and Models.} 
We conduct experiments on three benchmark datasets, including CIFAR-10~\cite{2009Learning}, CIFAR-100~\cite{2009Learning} and Tiny ImageNet~\cite{le2015tiny}. Specifically, CIFAR-10~\cite{2009Learning} contains 10 classes with 60,000 color images and the size of each image is ${32\times 32 \times 3}$. There are 50,000 images for training and 10,000 images for testing. CIFAR-100~\cite{2009Learning} has 100 classes, each of them containing 500 training images and 100 testing images. The size of an image in CIFAR-100 is the same as that in CIFAR-10~\cite{2009Learning}. Tiny ImageNet~\cite{le2015tiny} is a subset of ImageNet~\cite{deng2009imagenet} which contains 200 classes, with 500 images per class for training, 50 images per class for validation, and 50 images per class for testing. The size of each image is ${64\times 64 \times 3}$. The model architectures that we adopted are PreAct-ResNet18~\cite{he2016identity} and VGG19-BN~\cite{simonyan2014very}. 
\paragraph{Attack Settings}
% \noindent\textbf{Attack Settings.} 
We compare the proposed method with seven current state-of-the-art (SOTA) backdoor attacks, which can be divided into four categories: 1) \textit{non clean-label with spatial-statistic trigger}, such as BadNets~\cite{gu2019badnets} and Blended~\cite{chen2017targeted}; 2) \textit{non clean-label with spatial-dynamic trigger}, like SSBA~\cite{li2021invisible} and Input-Aware~\cite{nguyen2020input}; 3) \textit{clean-label with spatial-statistic trigger}, like SIG~\cite{barni2019new}; 4) \textit{non clean-label with frequency-statistic trigger}, including LF~\cite{zeng2021rethinking} and WABA~\cite{drager2022backdoor}. To verify the effectiveness of our method, we compare the attack performance with the SOTA attacks under different poisoning ratios, ranging from $0.004\%$ to $1\%$. It is worth noting that $0.004\%$ means that there are only 2 poisoned samples in the training dataset of CIFAR-10~\cite{2009Learning} and CIFAR-100~\cite{2009Learning}, and 4 poisoned samples in the training dataset of Tiny ImageNet~\cite{le2015tiny}. 
\paragraph{Defense Settings}
% \noindent\textbf{Defense Settings.}
We validate the performance of our method against multiple popular backdoor defense and detection methods. There are three backdoor detection methods (\textit{e.g.} AC~\cite{chen2018detecting}, SCAn~\cite{tang2021demon}, and STRIP~\cite{gao2019strip}.) and five SOTA backdoor defense methods (\textit{e.g.} CLP~\cite{zheng2022data}, FT, I-BAU~\cite{zeng2021adversarial}, NAD~\cite{li2021neural}, and NC~\cite{wang2019neural}.) are considered. For the detection methods, SCAn~\cite{tang2021demon} and STRIP~\cite{gao2019strip}, which assume that a detector can access a small set of benign samples, we assume the number of benign samples for each class to be 10, as recommended in these works. For the defense methods, we follow the default configuration used in BackdoorBench~\cite{wu2022backdoorbench,wu2023defenses} for a fair comparison. 
\begin{figure}[htbp]
\centering
\includegraphics[width=3.4in]{figures/selected_regions2.pdf}
\caption{The selected regions for CIFAR-10, CIFAR-100, and Tiny ImageNet, respectively.}
\label{selected region}
\end{figure}
% \noindent\textbf{Details of WPDA.}
\paragraph{Details of WPDA}
According to the description of WPDA shown in Sec. \ref{Method}, we will provide more details about the decomposition level of dataset, the selection of the poisoning regions, and the design of the trigger. 
\begin{enumerate}
    \item Dataset Decomposition.
% \textbf{1)}  Dataset Decomposition. 
% \textit{1) Dataset Decomposing:} 
Datasets with large volumes and numerous categories are often complex, requiring detailed decompositions to achieve effectiveness at extremely low poisoning ratios. Hence, in the experiment, we perform a 2-level WPD on CIFAR-10, while CIFAR-100 and Tiny ImageNet undergo a 3-level WPD.
% Based on the observation, datasets with large volumes and numerous categories  often require more levels of WPD to achieve effectiveness and stealthiness at extremely low poisoning ratios. 
\item Poisoning Regions Selection.
% \textbf{2)} Poisoning Regions Selection. 
% \textit{2) Poisoning Regions Selection:} 
Based on the analysis in Sec.~\ref{Analysis on dataset}, 
% the poisoning regions are those that have large information except the lowest frequency region, which means poisoning regions are different for these datasets. 
$4^{N-1}$ key poisoning regions of sub-spectrograms are selected as the poisoning regions (except the lowest frequency region in the spectrogram). We highlight the selected regions in Fig.~\ref{selected region}, in which it can be seen that there are four regions chosen in CIFAR-10 and 16 regions in CIFAR-100 and Tiny ImageNet. 
% \textbf{3)} Trigger Design. 
% \textit{3) Trigger Design:} 
\item Trigger Design.
In the following experiment, 
% we extract the contents in the poisoning frequency regions of a ``Hello Kitty'' image to serve as the trigger.
we select ``Hello Kitty'' image as the trigger.
For different datasets, the trigger information intensity $k$ in the poisoned training samples is altering, such as $k=6$ in CIFAR-10, $k=8$ in CIFAR-100, and $k=7$ in Tiny ImageNet. The values of the trigger information intensity $k'$ in the poisoned testing samples for different datasets can be referred to Tab.~\ref{test-value}, and the original information intensity $\alpha$ is 1.
\end{enumerate}
\paragraph{Evaluation Metrics}
% \noindent\textbf{Evaluation Metrics.} 
To evaluate the attack performance of our proposed method, we adopt two metrics: Clean Accuracy (C-Acc), defined as the prediction accuracy on all benign testing samples by the trained model, and Attack Success Rate (ASR), which measures the accuracy of poisoned testing samples being correctly predicted as the target class. The higher C-Acc and higher ASR imply better attack performance. Furthermore, to assess the performance of detection methods, we utilize three metrics: True Positive Rate (TPR), False Positive Rate (FPR), and Weighted F1 Score ($F_1^{\omega} = \frac{2TP}{2TP+FP+\omega FN'} $) used in ~\cite{yuan2023activation}. TPR reflects the accuracy with which detection methods identify poisoned samples, while FPR indicates the rate at which benign samples are mistakenly classified as poisoned. $F_1^{\omega}$ is one variant of $F_1$ score, which quantifies the detection method's ability to accurately classify poisoned samples while minimizing the misclassification of benign samples.
\input{tables/values_of_k}
\input{tables/experiment_attack_cifar10}
\subsection{Attack Performance of WPDA}
\label{Attack Performance on WPDA}
% \noindent\textbf{Evaluations on CIFAR-10}.
\paragraph{Evaluations on CIFAR-10}
Tab.~\ref{attack_result_CIFAR-10} illustrates the attack performance of the compared attack methods and our method on CIFAR-10 with various poisoning ratios. It is evident that other attacks cannot achieve good attack performance under the extremely low poisoning ratio of $0.004\%$. In this situation, the highest ASR achieved by Input-Aware is $12.36\%$ on Preact-ResNet18 and $10.19\%$ on VGG19-BN, respectively. In contrast, WPDA can achieve ASRs of $98.12\%$ on Preact-ResNet18 and $77.50\%$ on VGG19-BN. As the poisoning ratio increases, there is a significant improvement in attack performance. WPDA can achieve ASRs of $100\%$ on Preact-ResNet18 and $99.99\%$ on VGG19-BN. From Tab.~\ref{attack_result_CIFAR-10}, it is also evident that one advantage of low poisoning ratio attacks is their minimal impact on clean accuracy. Moreover, the C-Acc of WPDA is the highest among the compared attacks at a poisoning ratio of $0.004\%$, reaching $94.03\%$ on Preact-ResNet18 and $92.49\%$ on VGG19-BN, respectively.
\paragraph{Evaluations on CIFAR-100}
% \noindent\textbf{Evaluations on CIFAR-100}.
From Tab.~\ref{attack_result_CIFAR-100}, we notice that the highest ASR achieved by the compared methods is $1.29\%$ on Preact-ResNet and $1.04\%$ on VGG19-BN, which underscores the challenge of successfully embedding a backdoor at a poisoning ratio of $0.004\%$. At the same poisoning ratio, the ASR of WPDA can reach $85.01\%$ on Preact-ResNet and $79.94\%$ on VGG19-BN, respectively. It can be seen that WPDA consistently outperforms other attacks at the previous four poisoning ratios, but is surpassed by WABA at $1\%$ poisoning ratio. However, poisoned samples generated by WPDA are more natural and less visible to the naked eyes than those generated by WABA.
\input{tables/experiment_attack_cifar100}
% \noindent\textbf{Evaluations on Tiny ImageNet}.
\paragraph{Evaluations on Tiny ImageNet}
The attack performance on Tiny ImageNet is shown in Tab.~\ref{attack_result_tiny}. Similar to CIFAR-100, the compared methods cannot achieve a high ASR on Tiny ImageNet at a $0.004\%$ poisoning ratio. However, WPDA can still achieve an $80.99\%$ ASR on PreAct-ResNet18 and $64.96\%$ ASR on VGG19-BN with only 4 poisoned samples, both far exceeding the values achieved by the compared methods. If the compared methods aim to achieve the same level of attack performance, they would need to poison a larger number of samples, such as 1,000 samples in the training dataset of Tiny ImageNet. Due to the limited number of samples in each class, we are unable to conduct SIG on this dataset, which is a clean-label attack and only injects the trigger to the target class. 
\vspace{-0.1cm}
\begin{figure}[htbp]
\centering
% \includegraphics[width=3.6in]
\includegraphics[width=8.85cm,height=2.9cm]{figures/poisoned_samples1.pdf}
\caption{Visualization of the poisoned samples in datasets.}
\label{poisoned-samples}
\end{figure}
\vspace{0.1cm}
% \noindent\textbf{In summary}, 
\paragraph{In summary}
% the above comparisons demonstrate the superior attack performance of WPDA to 7 SOTA attacks, especially at low poisoning ratios.
The above comparisons demonstrate the superior attack performance of WPDA compared to 7 SOTA attacks, especially at low poisoning ratios.
Fig.~\ref{poisoned-samples} shows the visualization of the poisoned samples on CIFAR-10, CIFAR-100 and Tiny ImageNet. Compared with other attack methods, 
Although the backdoor samples based on WPDA method is not the most natural to the original image in visual, WPDA balances the effectiveness of the backdoor attack and the naturalness of the samples at a very low poisoning ratio.
\input{tables/experiment_attack_tiny}
\subsection{Detection Performance of WPDA}
\label{Detection Performance on WPDA}
% To evaluate the performance of WPDA against current detection methods, we applied three detectors to WPDA across three datasets and two models, using five different poisoning ratios. The results are shown in Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg}. 
%After the detection process was completed, we re-evaluated the effectiveness of our attack method. Specifically, we retrained the model using the samples reserved by the detectors, applying the same training hyper-parameters as before. The result of retraining is provided in \red{Tab.xxx}.
\paragraph{Evaluations on AC}
% leverages activation clustering to detect backdoor attacks. 
The core principle of AC lies in the observation that poisoned training samples activate specific neurons that are different from those activated by benign training samples. By leveraging activation clustering, samples are divided into two clusters, and the smaller one is regarded as poisoned.
Tab.~\ref{detection_result_pre} indicates that AC fails to correctly identify poisoned training samples, which is because the number of poisoned training samples is too small to be recognized as a distinct cluster by AC. Meanwhile, the activations of some benign samples are incorrectly divided into two clusters, with the smaller one being misidentified as poisoned. 
Tab.~\ref{detection_result_vgg} shows that, when the poisoning ratio is less than 0.1\%, the results are similar to those in Tab.~\ref{detection_result_pre}, successfully evading detection. 
% Considering CIFAR-10, with a poisoning ratio is 1\% trained on VGG19-BN,
Considering CIFAR-10, AC achieve 99.40\% TPR and 7.31\% FPR as the poisoning ratio increases to 1\%. These results indicate that AC's detection performance is influenced not only by the dataset and the model architectures but also by the poisoning ratios, with a particular proficiency in detecting backdoor attacks at higher poisoning ratios.
% In other words, As the poisoning ratio increases, the risk of detection also rises.
% From Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg}, we notice that AC fails to correctly identify poisoned samples in the training datasets when the poisoning ratio is less than $1\%$ across both model structures. Indeed, AC has misclassified many benign samples as poisoned; for instance, it exhibits a $11.31\%$ FPR in CIFAR-10 at a $0.05\%$ poisoning ratio. We conjecture that this is because the number of poisoned samples is too small to be recognized as a distinct cluster by AC. Meanwhile, the activations of some benign samples are incorrectly divided into two clusters, with the smaller one being misidentified as poisoned. When the poisoning ratio is $1\%$, AC can achieve $99.40\%$ TPR and $7.31\%$ FPR on CIFAR-10 trained by VGG19-BN. 
\paragraph{Evaluations on SCAn}
% \noindent\textbf{Evaluations on SCAn.}
SCAn leverages a statistical analysis method based on feature representations, identifying poisoned classes and poisoned training samples by examining whether their distribution aligns with a mixture of normal distributions. Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg} demonstrate that SCAn’s effectiveness in detecting poisoned training samples is hindered by low poisoning ratios, but its performance significantly improves as the poisoning ratios rises. For instance, on Tiny ImageNet, SCAn achieves a TPR of 99.90\% and 99.10\% TPR when trained on PreAct-ResNet18 and VGG19-BN, respectively. On CIFAR-10, SCAn achieves a 98.40\% TPR when trained on VGG19-BN. These observations illustrate that: 1) at extremely low poisoning ratios, the EM algorithm utilized by SCAn fails to recognize the target class as a mixed distribution; 2) the effectiveness of this detection method depends on the activations extracted by the models.
% SCAn, another detection method based on activations, 
% is found to be ineffective at all poisoning ratios on PreAct-ResNet18. However, when applied to VGG19-BN, SCAn successfully detects poisoned samples, achieving a 98.40\% TPR on CIFAR-10 and 99.10\% TPR on Tiny ImageNet at a 1\% poisoning ratio. Yet, it fails to identify poisoned samples at the previous four poisoning ratios with VGG19-BN. These observations illustrate that: 1) at extremely low poisoning ratios, the EM algorithm utilized by SCAn fails to recognize the target class as a mixed distribution; 2) the effectiveness of this detection method depends on the activations extracted by the models.
\paragraph{Evaluations on STRIP}
% \noindent\textbf{Evaluations on STRIP}. 
STRIP is a detection method based on the perturbation of inputs. The principle behind this detection method is that the predictions on perturbed poisoned samples are more consistent than the predictions on benign samples. Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg} demonstrate that there is a notable difference in the detection performance of STRIP between PreAct-ResNet18 and VGG19-BN. This discrepancy can be primarily attributed to the inherent differences in model architectures. Each model possesses its unique architecture and learning capabilities, leading to disparities in performance even when confronted with identical datasets. However, the trend presented by the models is consistent, \textit{i.e.}, the TPR of STRIP on all three datasets rises as the poisoning ratios increases. Considering CIFAR-10, with a poisoning ratio is 0.004\%, Tab.~\ref{detection_result_pre} reports a TPR of 50.00\%. A further analysis indicates that among the 50,000 training samples, STRIP identifies 6,637 as suspicious, while only two poisoned training samples actually exist. This implies that STRIP successfully detect only one of the backdoor samples. After discarding all the suspicious samples and re-training, the resulting C-Acc of 92.72\% and ASR of 98.54\% demonstrate that the attack remains effective.

\input{tables/experiment_detection1}
\input{tables/experiment_detection2}
% \vspace{-1mm}
\paragraph{In summary}
% \noindent\textbf{In summary,} 
% based on the above results, it is observed that attacks with low poisoning ratios are more stealthy against backdoor detection methods than those with high poisoning ratios. 
Based on the above results, it is evident that attacks with high poisoning ratios are more easily to be detected than those with low poisoning ratios. At low poisoning ratios, a few number of poisoned training samples can make anomalous behaviour relatively undetectable.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=3.7in]{figures/cifar100_tiny_clp_nc1.pdf}
\caption{t-SNE on mixed testing samples after defenses. One color corresponds to one class. We randomly select benign testing samples from 10 classes in the total classes, which also includes benign testing samples in the target class. The black circles represent the poisoned testing samples in target class. (Left: t-SNE on CIFAR-100 after CLP, target class is `Apple’, Right: t-SNE on Tiny ImageNet after NC, target class is`Goldfish'.)
}
\label{cifar100_tiny_clp_nc}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering  %图片全局居中
    \subfigure[PreAct-ResNet18]{
    \includegraphics[width=8.88cm,height =4.1cm]{figures/cifar10_preactresnet18_1_.pdf}}
    \label{CIFAR-10_PreAct-ResNet18}
    \subfigure[VGG19-BN]{
    \includegraphics[width=8.88cm,height =4.1cm]{figures/cifar10_vgg19_bn_1_.pdf}}
    \label{CIFAR-10_vgg_bn}
\caption{CIFAR-10 backdoor attack performance against 5 defense methods. Each sub-plot corresponds to one defense method. In each sub-pot, each pillar in the histogram indicates the ASR value of one attack method, and the C-Acc values are represented by dotted curves.}
\label{cifar10-defense}
\end{figure*}
\subsection{Defense Performance of WPDA}
\label{Defense Performance on WPDA}
In the following, we evaluate the attack performance of WPDA and other attacks under 5 SOTA backdoor defense methods.
\paragraph{Evaluations on CIFAR-10}
% \textbf{Evaluations on CIFAR-10}.
Fig.~\ref{cifar10-defense} illustrates the performance of 7 SOTA attack methods and WPDA against 5 SOTA defense methods. Compared with other attack methods, WPDA shows stable performance after various defense methods at every poisoning ratio. 
Besides, backdoor attacks at low poisoning ratios are more stable than those at high poisoning ratios in some cases. For example, the ASR of attack methods such as Blended, Input-Aware and WPDA at 0.05\% poisoning ratio decays less than that at 0.1\% poisoning ratios after I-BAU on PreAct-ResNet18, Input-Aware and WABA on VGG19-BN have the same performance after NC. 
\begin{figure*}[t]
\centering  %图片全局居中
    \subfigure[PreAct-ResNet18]{
    \includegraphics[width=8.88cm,height =4.1cm]{figures/cifar100_preactresnet18_1_.pdf}}
    \label{cifar100_preactresnet18}
    \subfigure[VGG19-BN]{
    \includegraphics[width=8.88cm,height =4.1cm]{figures/cifar100_vgg19_bn_1_.pdf}}
    \label{cifar100_vgg19_bn}
\caption{CIFAR-100 backdoor attack performance under different defenses. 
Each sub-plot corresponds to one defense method. In each sub-pot, each pillar in the histogram indicates the ASR value of one attack method, and the C-Acc values are represented by dotted curves.}
\label{cifar100-defense}
\end{figure*}
\paragraph{Evaluations on CIFAR-100}
Fig.~\ref{cifar100-defense} illustrates that WPDA at low poisoning ratios shows advantages after various defense methods. As for PreAct-ResNet18, WPDA achieves optimal performance compared with other attacks at low poisoning ratios. WPDA at low poisoning ratios is even more stable than WPDA at high poisoning ratios, such as against CLP, I-BAU and NC. As for VGG19-BN, results illustrate that attacks at high poisoning ratios increase the risk of success against defenses, \textit{i.e.}, a significant decay of ASR at high poisoning ratios. Fig.~\ref{cifar100_tiny_clp_nc}(Left) shows the t-SNE on the mixed testing samples of CIFAR-100 after CLP. The poisoned testing samples are clearly separated from benign testing samples in the target class after CLP, which means the model effectively captures the channels related to the backdoor, causing the attack to fail. However, lots of benign samples in other classes overlap in the feature space, which results in a significant drop of the model's accuracy on benign testing samples.
% \vspace{-0.6cm}
\begin{figure*}[t]
\centering  %图片全局居中
    \subfigure[PreAct-ResNet18]{
    \label{tiny_PreAct-ResNet18}
    \includegraphics[width=8.7cm,height =4.0cm]{figures/tiny_preactresnet18_1_.pdf}}
    \subfigure[VGG19-BN]{
    \label{tiny_vgg_bn}
    \includegraphics[width=8.7cm,height =4.0cm]{figures/tiny_vgg19_bn_.pdf}}
\caption{Tiny ImageNet~\cite{le2015tiny} backdoor attack performance under different defenses on PreAct-ResNet18~\cite{he2016identity}. Each sub-plot corresponds to one defense method. In each sub-pot, each pillar in the histogram indicates the ASR value of one attack method, and the C-Acc values are represented by dotted curves.}
\label{tiny-attack}
\end{figure*}\\
\paragraph{Evaluations on Tiny ImageNet}
Fig.~\ref{tiny-attack} illustrates WPDA trained by Tiny ImageNet is very stable, not only achieving successful attacks, but remaining effective after the defenses, even at low poisoning ratios. The results also show that the backdoor attacks at low poisoning ratios increase the stealth of the attack, for example, WPDA's ASR decay at low poisoning ratios is less than that at high poisoning ratios against I-BAU on both PreAct-ResNet18 and VGG19-BN. Not only WPDA, Input-Aware trained on PreAct-ResNet18 and VGG19-BN also shows the same performance against NC.
What needs to be analysed in particular is the performance of WPDA at 0.01\% poisoning ratio after AC. Fig.~\ref{cifar100_tiny_clp_nc}(Right) illustrates that the poisoned testing samples are effectively separated from the samples in the target class. Although the backdoor effect is effectively mitigated by pruning neurons that are highly correlated with the backdoor, the accuracy of the benign testing samples drops substantially. As for NAD, when the model's attention is shifted, few poisoned training samples cannot promote the model to learn the trigger information effectively, leading to a drop in ASR. Although the effectiveness of WPDA is influenced, the accuracy of the model on benign testing samples decays a lot after NC.\
\begin{figure}[H]
\centering
\includegraphics[width=3.65in]{figures/tiny_nad1.pdf}
\caption{t-SNE on mixed testing samples of Tiny ImageNet after NAD. NAD remove the backdoor effect of WPDA but the accuracy of benign samples are influenced. (Target Class is `Goldfish')}
\label{tiny-nad}
\end{figure}
\paragraph{In summary}
Most defense methods are difficult to defend against backdoor attacks with low poisoning ratios, which indicates that it is necessary to explore backdoor attacks at low poisoning ratios. Compared with 7 SOTA attack method, WPDA shows more stable and stealthy performance, especially at low poisoning ratios.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analyses}
\label{tsne-kde}
\subsection{Visualization on t-SNE}
Fig.~\ref{tsne-01-all-attack} shows the t-SNE of 7 SOTA attacks and WPDA on PreAct-ResNet18 trained by CIFAR-10 at 1\% poisoning ratio. 7 SOTA attacks and WPDA achieve high ASR at 1\% poisoning ratio, and the poisoned training samples are close to the benign samples in the target class and the poisoned testing samples, which means that the features extracted by the model from those samples exhibit significant similarity. We conclude that the model effectively learns the trigger rather than memorizing the poisoned training samples. In Fig.~\ref{tsne-00004-all-attack}, as for BadNets, Blended, Input-Aware, SIG, SSBA, LF and WABA, the poisoned training samples are close to the benign samples in the target class, while the poisoned testing samples are evenly distributed across the classes. In other words, the models based on these attack methods only memorize the poisoned training samples rather than learning the features of the trigger, which results in the backdoor not being activated when the poisoned testing samples are used as inputs. However, the poisoned training samples generated by WPDA are not only close to the samples in the target class but also to the poisoned testing samples in the feature space, which is consistent with the performance of attacks at 1\% poisoning ratio. In summary, WPDA precisely injects trigger information into the key frequency regions, prompting the model to effectively learn the trigger information even at low poisoning ratios. 
\vspace{-0.5cm}
\begin{figure*}[t]
\centering  %图片全局居中
    \subfigure[0.004\% poisoning ratio]{
    \label{tsne-00004-all-attack}
\includegraphics[width=8.7cm,height=4.1cm]{figures/tsne1.jpg}}  
    % =4.1cm]{figures/tsne00004_11.png}}
    \subfigure[1\% poisoning ratio]{
    \label{tsne-01-all-attack}
\includegraphics[width=8.7cm,height=4.1cm]{figures/tsne2.jpg}} 
    % =4.1cm]{figures/tsne01_1.png}}
\centering 
\caption{t-SNE about 7 SOTA attack methods and WPDA at 0.004\% and 1\% poisoning ratios.}
\label{}
\end{figure*}
\subsection{{Visualization on \texorpdfstring{$l_2$}-distance KDE}}
Kernel Density Estimation (KDE) is a non-parametric statistical method for estimating the Probability Density Function (PDF) that can be used to describe the distribution of data~\cite{gramacki2018nonparametric}. Specifically, KDE is a measure of estimated probability density defined by a kernel function near each data point in the dataset. In KDE, we usually choose a kernel function and a bandwidth parameter to define the similarity between each data point in the dataset and other data points, usually using the Gaussian kernel function, \etc~\\
\hspace*{0.15cm}
To further verify the effectiveness of the WPDA attack, we conduct $l_2$-distance KDE visualization analyses on PreAct-ResNet18 trained by CIFAR-10 at different poisoning ratios. At first, we extract the features of poisoned samples from the `linear' layer in PreAct-ResNet18 and calculate the $l_2$ distance between each poisoned training sample and each poisoned testing sample, then we can obtain multiple lists of $l_2$-distance between each poisoned training sample and all poisoned testing samples, where the number of lists is equal to the number of poisoned training samples and the length of each list is equal to the number of poisoned testing samples. 
Then average the multiple lists of $l_2$-distance and conduct KDE visualization. 

In Fig.~\ref{kde}, the horizontal axis represents the average $l_2$ distance between the poisoned training samples and the poisoned testing samples, and the vertical axis represents the density of each $l_2$-distance value. The $l_2$-distance with a large value means that the features extracted by the model from the poisoned training samples have a large variability from the features extracted from the poisoned testing samples. It is much difficult for the model to predict the poisoned testing samples as target class.
At 0.004\% poisoning ratio, the $l_2$-distance in WPDA are mainly concentrated in small values, which indicates that the features extracted by the model from the poisoned testing samples are similar to those extracted in the poisoned training samples. While, for other attacks, the features extracted by the model from the poisoned testing samples differ from those extracted from the poisoned training samples. As the poisoning ratios increases, $l_2$-distance value in each attack decreases and concentrates gradually, indicating that the model gradually learns the trigger information.
\begin{figure}[!ht]
\centering  %图片全局居中
% \captionsetup[subfigure]{labelformat=empty} 
    {
    \includegraphics[width=1.65in]{figures/kde_all_attack_00004_1.pdf}}
    \label{kde-00004}
% \captionsetup[subfigure]{labelformat=empty} 
    {
    \includegraphics[width=1.65in]{figures/kde_all_attack_01_1.pdf}}
    \label{kde-01}
\caption{$l_2$-distance KDE on PreAct-ResNet18 trained by CIFAR-10 at 0.004\% poisoning ratio (left) and 1\% poisoning ratio (right).}
\label{kde}
% \vspace{-0.5cm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

Section~\ref{Qualitative Analysis}c has demonstrated that models exhibit generalization ability. To confirm our conclusions, we conduct $l_2$-distance KDE visualization by modifying original information intensities $\alpha$ and trigger information intensities $k'$ of the poisoned testing samples.
Fig.~\ref{kde-alpha} shows the $l_2$-distance KDE visualization under different original information intensities $\alpha$. With the increase of the intensity of original information $\alpha$, the $l_2$ distance in feature space between the poisoned testing samples and the poisoned training samples gradually increases. As a result, the original information has a negative effect on the backdoor model, but we can rely on the model's generalization ability to activate the backdoor when the prominence of the trigger is stronger than that of the original information.
Fig.~\ref{kde-k'} shows the $l_2$-distance KDE visualization under different trigger information intensities  $k'$. The increase of the trigger information intensity $k'$ can promote the backdoor model to capture the trigger information, which is positive for the activation of the backdoor.

\begin{figure}[!ht]
\centering  %图片全局居中
    \subfigure[$l_2$-distance KDE under different original information intensities $\alpha$]{
    \label{kde-alpha}
    \includegraphics[width=1.6in]{figures/tsne_WPDA_alpha_00004_.pdf}}
    \subfigure[$l_2$-distance KDE under different trigger information intensities $k'$]{
    \label{kde-k'}
    \includegraphics[width=1.6in]{figures/tsne_WPDA_k1_00004_.pdf}}
\caption{$l_2$-distance KDE on PreAct-ResNet18 trained by CIFAR-10 at 0.004\% ratio.}
\label{kde-generation}
\end{figure}



% Section~\ref{stealthiness of trigger information} has demonstrated that the model is generalizable. 
% Fig.~\ref{memorizing_pre} shows the the feature distribution under different original information intensities. Both on PreAct-ResNet18 and VGG19-BN, with the increase of the intensity of original information, the difference in feature distribution between the testing samples and the training samples becomes more obvious. As a result, the original information has a negative effect on the backdoor model to activate the backdoor, and WPDA is to promote the model to learn trigger information rather than memorizing backdoor samples. 
% % Therefore, we conclude that the model effectively learns the trigger, rather than memorizing the poisoned samples.
% Fig.~\ref{KDE-PreAct-ResNet18-others} shows the KDE distribution of 7 SOTA methods and WPDA on PreAct-ResNet18 trained by CIFAR-10 at 0.004\% poisoning ratio. As for BadNets, Blended, Input-Aware, SIG, SSBA, LF and WABA, the distribution of the average features of the poisoned training samples is quite different from that of the poisoned testing samples. In other words, the model based on these attack methods only remembers the poisoned training samples rather than learn the characteristics of the trigger, which causes the backdoor to not be activated. 
% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=6in]{figures/memorizing_alpha1.png}
% \caption{The KDE visualization based on our method of CIFAR-10 with 0.004\% poisoning ratio. We modify the intensity of original image information to  (First row: Model PreAct-ResNet18; Second row: Model VGG19-BN).}
% \label{memorizing_pre}
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=5in]{figures/tsne00004_1.png}
% \caption{The KDE visualization of different attack methods based on CIFAR-10 with 0.004\% poisoning ratio trained by PreAct-ResNet18.}
% \label{KDE-PreAct-ResNet18-others}
% \end{figure*}

                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     

==> tip/5_experiment_new.tex <==
\section{Experiments}
\label{Experiment}
\subsection{Experiment Settings}
\paragraph{\textbf{Datasets and Models}}
% \noindent\textbf{Datasets and Models.} 
We conduct experiments on three benchmark datasets, including CIFAR-10~\cite{2009Learning}, CIFAR-100~\cite{2009Learning} and Tiny ImageNet~\cite{le2015tiny}. Specifically, CIFAR-10~\cite{2009Learning} contains 10 classes with 60,000 color images and the size of each image is ${32\times 32 \times 3}$. There are 50,000 images for training and 10,000 images for testing. CIFAR-100~\cite{2009Learning} has 100 classes, each of them containing 500 training images and 100 testing images. The size of an image in CIFAR-100 is the same as that in CIFAR-10~\cite{2009Learning}. Tiny ImageNet~\cite{le2015tiny} is a subset of ImageNet~\cite{deng2009imagenet} which contains 200 classes, with 500 images per class for training, 50 images per class for validation, and 50 images per class for testing. The size of each image is ${64\times 64 \times 3}$. The model architectures that we adopted are PreAct-ResNet18~\cite{he2016identity} and VGG19-BN~\cite{simonyan2014very}. 
\paragraph{\textbf{Attack Settings}}
We compare the proposed method with seven current state-of-the-art (SOTA) backdoor attacks, which can be divided into four categories: 1) \textit{non clean-label with spatial-static trigger}, such as BadNets~\cite{gu2019badnets} and Blended~\cite{chen2017targeted}; 2) \textit{non clean-label with spatial-dynamic trigger}, like SSBA~\cite{li2021invisible} and Input-aware~\cite{nguyen2020input}; 3) \textit{clean-label with spatial-static trigger}, like SIG~\cite{barni2019new}; 4) \textit{non clean-label with frequency-statistic trigger}, including LF~\cite{zeng2021rethinking} and WABA~\cite{drager2022backdoor}. To verify the effectiveness of our method, we compare the attack performance with the SOTA attacks under different poisoning ratios, ranging from $0.004\%$ to $0.1\%$. It is worth noting that $0.004\%$ means that there are only 2 poisoned samples in the training dataset of CIFAR-10~\cite{2009Learning} and CIFAR-100~\cite{2009Learning}, and 4 poisoned samples in the training dataset of Tiny ImageNet~\cite{le2015tiny}. 
\paragraph{\textbf{Defense Settings}}
We validate the performance of our method against multiple popular backdoor defense and detection methods. There are three backdoor detection methods (\textit{e.g.} AC~\cite{chen2018detecting}, SCAn~\cite{tang2021demon}, and STRIP~\cite{gao2019strip}.) and five SOTA backdoor defense methods (\textit{e.g.} CLP~\cite{zheng2022data}, FT, I-BAU~\cite{zeng2021adversarial}, NAD~\cite{li2021neural}, and NC~\cite{wang2019neural}.) are considered. For the detection methods, SCAn~\cite{tang2021demon} and STRIP~\cite{gao2019strip}, which assume that a detector can access a small set of benign samples, we assume the number of benign samples for each class to be 10, as recommended in these works. For the defense methods, we follow the default configuration used in BackdoorBench~\cite{wu2022backdoorbench,wu2023defenses} for a fair comparison. 
\begin{figure}[htbp]
\centering
\includegraphics[width=3.4in]{figures/selected_regions2.pdf}
\caption{The selected regions for CIFAR-10, CIFAR-100, and Tiny ImageNet, respectively.}
\label{selected region}
\end{figure}
\paragraph{\textbf{Details of WPDA}}
According to the description of WPDA shown in Sec.~\ref{Method}, we will provide more details about the decomposition level of dataset, the selection of the poisoning regions, and the design of the trigger. 
\begin{enumerate}
    \item \textbf{Dataset Decomposition}.
Datasets with large volumes and numerous categories are often complex, requiring detailed decompositions to achieve effectiveness at extremely low poisoning ratios. Hence, in the experiment, we perform a 2-level WPD on CIFAR-10, while CIFAR-100 and Tiny ImageNet undergo a 3-level WPD.
\item \textbf{Poisoning Regions Selection}.
Based on the analysis in Sec.~\ref{Analysis on dataset}, $4^{N-1}$ key poisoning regions of sub-spectrograms are selected as the poisoning regions (except the lowest frequency region in the spectrogram). We highlight the selected regions in Fig.~\ref{selected region}, in which it can be seen that there are 4 regions chosen in CIFAR-10 and 16 regions in CIFAR-100 and Tiny ImageNet. 
% \textbf{3)} Trigger Design. 
% \textit{3) Trigger Design:} 
\item \textbf{Trigger Design}.
In the following experiment, we select ``Hello Kitty'' image derived from Blended as the trigger.
For different datasets, the trigger information intensity $k$ in the poisoned training samples is altering, such as $k=6$ in CIFAR-10, $k=8$ in CIFAR-100, and $k=7$ in Tiny ImageNet. The values of the trigger information intensity $k'$ in the poisoned testing samples for different datasets can be referred to Tab.~\ref{test-value}, and the original information intensity $\alpha$ is 1.
\end{enumerate}
\input{tables/values_of_k}
\paragraph{\textbf{Evaluation Metrics}}
To evaluate the attack performance of our proposed method, we adopt two metrics: Clean Accuracy (C-Acc), defined as the prediction accuracy on all benign testing samples by the trained model, and Attack Success Rate (ASR), which measures the accuracy of poisoned testing samples being correctly predicted as the target class. The higher C-Acc and higher ASR imply better attack performance. Furthermore, to assess the performance of detection methods, we utilize three metrics: True Positive Rate (TPR), False Positive Rate (FPR), and Weighted F1 Score ($F_1^{\omega} = \frac{2TP}{2TP+FP+\omega FN'} $) used in ~\cite{yuan2023activation}. TPR reflects the accuracy with which detection methods identify poisoned samples, while FPR indicates the rate at which benign samples are mistakenly classified as poisoned. $F_1^{\omega}$ is one variant of $F_1$ score, which quantifies the detection method's ability to accurately classify poisoned samples while minimizing the misclassification of benign samples.
\input{tables/experiment_attack_cifar10_new}
\subsection{Attack Performance of WPDA}
\label{Attack Performance on WPDA}
\paragraph{\textbf{Evaluations on CIFAR-10}}
Tab.~\ref{attack_result_CIFAR-10} illustrates the attack performance of the compared attack methods and our method on CIFAR-10 with various poisoning ratios. It is evident that other attacks cannot achieve good attack performance under the extremely low poisoning ratio of $0.004\%$. In this situation, the highest ASR achieved by Input-aware is $12.36\%$ on Preact-ResNet18 and $10.19\%$ on VGG19-BN, respectively. In contrast, WPDA can achieve ASRs of $98.12\%$ on Preact-ResNet18 and $77.50\%$ on VGG19-BN. As the poisoning ratio increases, there is a significant improvement in attack performance. WPDA can achieve ASRs greater than $99\%$ on both Preact-ResNet18 and VGG19-BN. Besides, it is also evident that one advantage of low poisoning ratio attacks is their minimal impact on clean accuracy. Moreover, the C-Acc of WPDA is the highest among the compared attacks at a poisoning ratio of $0.004\%$, reaching $94.03\%$ on Preact-ResNet18 and $92.49\%$ on VGG19-BN, respectively.
% \input{tables/experiment_attack_cifar10}

\paragraph{\textbf{Evaluations on CIFAR-100}}
From Tab.~\ref{attack_result_CIFAR-100}, we note that the highest ASR achieved by the compared methods is $1.29\%$ on Preact-ResNet and $1.04\%$ on VGG19-BN, which underscores the challenge of successfully embedding a backdoor at a poisoning ratio of $0.004\%$. At the same poisoning ratio, the ASR of WPDA can reach $85.01\%$ on Preact-ResNet and $79.94\%$ on VGG19-BN, respectively. As the poisoning ratio increases, the ASR of most attack methods exhibits an upward trend. While, our method demonstrates a slight decrease in ASR at a poisoning rate of 0.1\% compared to 0.05\%, which is attributed our dynamic adjustment of the trigger intensity $k'$ in poisoned testing samples based on the poisoning ratios, setting a small $k'$ value on a high poisoning ratio. Despite this adjustment causing a slight fluctuation in ASR, our method still achieves the best overall performance compared to the other 7 attack methods. 
% It can be seen that WPDA consistently outperforms other attacks at all the poisoning ratios, but is surpassed by WABA at $1\%$ poisoning ratio. However, poisoned samples generated by WPDA are more natural and less visible to the naked eyes than those generated by WABA.
% \input{tables/experiment_attack_cifar100}
\input{tables/experiment_attack_cifar100_new}
\paragraph{\textbf{Evaluations on Tiny ImageNet}}
The attack performance on Tiny ImageNet is shown in Tab.~\ref{attack_result_tiny}. Similar to CIFAR-100, the 7 compared attack methods cannot achieve a high ASR on Tiny ImageNet at $0.004\%$ poisoning ratios. However, WPDA can still achieve an $80.99\%$ ASR on PreAct-ResNet18 and $64.96\%$ ASR on VGG19-BN with only 4 poisoned samples, both far exceeding the values achieved by the compared methods. If the compared methods aim to achieve the same level of attack performance, they would need to poison a larger number of samples. At other poisoning ratios, our method continues to outperform the 7 compared attack methods, achieving the best performance.
% \input{tables/experiment_attack_tiny}
\input{tables/experiment_attack_tiny_new}
\paragraph{\textbf{In summary}}
The performance of other attack methods underscores the significant challenges associated with backdoor attacks under low poisoning ratios. Our method strategically selects the poisoning frequency regions based on the characteristics of the dataset, enhancing the efficiency of the attack and achieving a high ASR even with only 2 poisoned training samples on CIFAR-10 and CIFAR-100, 4 poisoned training samples on Tiny ImageNet. Besides, poisoned testing samples maintain the naturalness (shown in Fig.~\ref{poisoned-samples}).
% The above comparisons demonstrate the superior attack performance of WPDA compared to 7 SOTA attacks, even at low poisoning ratios.
% Fig.~\ref{poisoned-samples} shows the visualization of the poisoned samples on CIFAR-10, CIFAR-100 and Tiny ImageNet. 
% Compared with other attack methods. 
% Although the backdoor samples based on WPDA method is not the most natural to the original image in visual, WPDA balances the effectiveness of the backdoor attack and the naturalness of the samples at a very low poisoning ratio.
\begin{figure}[htbp]
\centering
% \includegraphics[width=3.6in]
\includegraphics[width=8.85cm,height=2.9cm]{figures/poisoned_samples1.pdf}
\caption{Visualization of the poisoned samples in datasets.}
\label{poisoned-samples}
\end{figure}
\subsection{Detection Performance of WPDA}
\label{Detection Performance on WPDA}
Due to the low ASR of the 7 compared attack methods compared at low injection ratios, we only evaluate the performance of WPDA on 3 detection methods. The performance on PreAct-ResNet18 is 
% similar to that on VGG19-BN, and the details on PreAct-ResNet18 are 
shown in Appendix~\ref{detection on pre}.
\paragraph{\textbf{Evaluations on AC}}
% leverages activation clustering to detect backdoor attacks. 
The core principle of AC lies in the observation that poisoned training samples activate specific neurons that are different from those activated by benign training samples. By leveraging activation clustering, samples are divided into two clusters, and the smaller one is regarded as poisoned.
Tab.~\ref{detection_result_vgg} indicates that AC fails to correctly identify poisoned training samples, which is because the number of poisoned training samples is too small to be recognized as a distinct cluster by AC. Meanwhile, the activations of some benign samples are incorrectly divided into two clusters, with the smaller one being misidentified as poisoned. These results indicate that WPDA can evade the detection of AC effectively.
% Tab.~\ref{detection_result_vgg} shows that, when the poisoning ratio is less than 0.1\%, the results are similar to those in Tab.~\ref{detection_result_pre}, successfully evading detection. 
% % Considering CIFAR-10, with a poisoning ratio is 1\% trained on VGG19-BN,
% Considering CIFAR-10, AC achieve 99.40\% TPR and 7.31\% FPR as the poisoning ratio increases to 1\%. These results indicate that AC's detection performance is influenced not only by the dataset and the model architectures but also by the poisoning ratios, with a particular proficiency in detecting backdoor attacks at higher poisoning ratios.

\paragraph{\textbf{Evaluations on SCAn}}
% \noindent\textbf{Evaluations on SCAn.}
SCAn leverages a statistical analysis method based on feature representations, identifying poisoned classes and poisoned training samples by examining whether their distribution aligns with a mixture of normal distributions.  As demonstrated in Tab.~\ref{detection_result_vgg}, the limited number of poisoned training samples poses a challenge for SCAn. With a negligible statistical footprint, these samples become difficult to identify through statistical analysis methods, hindering the effectiveness of SCAn at low poisoning ratios. 
% Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg} demonstrate that SCAn’s effectiveness in detecting poisoned training samples is hindered by low poisoning ratios, but its performance significantly improves as the poisoning ratios rises. For instance, on Tiny ImageNet, SCAn achieves a TPR of 99.90\% and 99.10\% TPR when trained on PreAct-ResNet18 and VGG19-BN, respectively. On CIFAR-10, SCAn achieves a 98.40\% TPR when trained on VGG19-BN. These observations illustrate that: 1) at extremely low poisoning ratios, the EM algorithm utilized by SCAn fails to recognize the target class as a mixed distribution; 2) the effectiveness of this detection method depends on the activations extracted by the models.

\paragraph{\textbf{Evaluations on STRIP}}
% \noindent\textbf{Evaluations on STRIP}. 
STRIP is a detection method based on the perturbation of inputs. The principle behind this detection method is that the predictions on perturbed poisoned samples are more consistent than the predictions on benign samples. Tab.~\ref{detection_result_vgg} demonstrates a positive correlation between the poisoning ratios and TPR. For instance, on CIFAR-10, with a poisoning ratio of 0.05\%, STRIP achieves a TPR of 32.00\%. This increases to 42.00\% when the poisoning ratio is doubled to 0.1\%. On Tiny ImageNet, STRIP achieves a TPR of 40.00\% and 70.00\% on 0.05\% and 0.1\% poisoning ratios, respectively. The results indicate that a large number of poisoned training samples has a higher risk of being detected by the detection method than a small number of poisoned training samples. A further analysis is shown in Fig.~\ref{STRIP detection vgg}, for attacks where STRIP successfully detects poisoned training samples, we conduct retraining experiments after removing all suspicious samples. The results indicate that STRIP fails to identify all poisoned training samples, so even if suspicious samples are removed, the remaining backdoor still works with a high ASR. Furthermore, on Tiny ImageNet, STRIP misidentifying some benign training samples as poisoned leads to an increase in the proportion of poisoned training samples, resulting in the elevated ASR.

% Tab.~\ref{detection_result_pre} and Tab.~\ref{detection_result_vgg} demonstrate that there is a notable difference in the detection performance of STRIP between PreAct-ResNet18 and VGG19-BN. This discrepancy can be primarily attributed to the inherent differences in model architectures. Each model possesses its unique architecture and learning capabilities, leading to disparities in performance even when confronted with identical datasets. However, the trend presented by the models is consistent, \textit{i.e.}, the TPR of STRIP on all three datasets rises as the poisoning ratios increases. Considering CIFAR-10, with a poisoning ratio is 0.004\%, Tab.~\ref{detection_result_pre} reports a TPR of 50.00\%. A further analysis indicates that among the 50,000 training samples, STRIP identifies 6,637 as suspicious, while only two poisoned training samples actually exist. This implies that STRIP successfully detect only one of the backdoor samples. After discarding all the suspicious samples and re-training, the resulting C-Acc of 92.72\% and ASR of 98.54\% demonstrate that the attack remains effective.
\input{tables/detection_VGG}
\begin{figure}[htbp]
\centering
% \includegraphics[width=3.6in]
\includegraphics[width=8.82cm,height=2.9cm]{figures/detection_retrain_vgg.pdf}
\caption{Results of STRIP retraining after removing suspicious samples on VGG19-BN.}
\label{STRIP detection vgg}
\end{figure}


\paragraph{\textbf{In summary}}
Based on the above results, it is evident that attacks with high poisoning ratios are more easily detected than those with low poisoning ratios. At low poisoning ratios, a small number of poisoned training samples can make anomalous behaviour relatively undetectable. WPDA not only achieves a high ASR even at a low poisoning ratio but also effectively evades detection methods.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Defense Performance of WPDA}
\label{Defense Performance on WPDA}
In the following, we evaluate the attack performance of WPDA and other attacks under 5 SOTA backdoor defense methods. The details on PreAct-ResNet18 are shown in Appendix~\ref{defense on pre}.
\paragraph{\textbf{Evaluations on CIFAR-10}}
% \textbf{Evaluations on CIFAR-10}.
Fig.~\ref{CIFAR-10_vgg_defense} illustrates the performance of 7 SOTA attack methods and WPDA against 5 SOTA defense methods. Compared with other attack methods, WPDA shows stable performance after various defense methods at every poisoning ratio. 
Besides, backdoor attacks at low poisoning ratios are more stable than those at high poisoning ratios in some cases. For instance, the ASR of attack methods such as Blended, Input-aware and WPDA at 0.05\% poisoning ratio decays less than that at 0.1\% poisoning ratios after 5 defense methods. 

 \begin{figure}[t]
\centering  %图片全局居中
    \subfigure[CIFAR-10]{ 
    \includegraphics[width=8.2cm,height =4.0cm]
    {figures/cifar10_vgg19_bn_2.pdf}
    \label{CIFAR-10_vgg_defense}}
    \subfigure[CIFAR-100]{
    \includegraphics[width=8.2cm,height =4.0cm]{figures/cifar100_vgg19_bn_2.pdf}
    \label{CIFAR-100_vgg_defense}}
    \subfigure[Tiny ImageNet]{
    \includegraphics[width=8.2cm,height =4.0cm]
    {figures/tiny_vgg19_bn_2.pdf}
    \label{tiny_vgg_defense}}
\caption{Results of 7 compared attack methods and WPDA against 5 defense methods on VGG19-BN, including CLP, FT, I-BAU, NAD and NC. Each sub-plot corresponds to one defense method. In each sub-plot, each bar in the histogram indicates the ASR value of one attack method, and the C-Acc values are represented by curves.}
\label{all-defense-vgg}
\end{figure}

\paragraph{\textbf{Evaluations on CIFAR-100}}
Fig.~\ref{CIFAR-100_vgg_defense} illustrates in most cases, WPDA maintains superior performance after 5 defense methods, especially at low poisoning ratios. Although WPDA exhibits a significant decline in ASR at 0.004\% poisoning ratio after CLP, the backdoor still works and outperforms other compared attack methods. Besides, the stability of attack methods at high poisoning ratios is weaker than that at low poisoning ratios. For instance, methods such as WPDA, Blended, and WABA exhibit a greater decline in ASR after defense methods such as CLP, NAD, NC at a 0.05\% poisoning ratio than at a 0.1\% poisoning ratio.
% Fig.~\ref{all-defense-vgg}(b) illustrates that WPDA at low poisoning ratios shows advantages after various defense methods. As for PreAct-ResNet18, WPDA achieves optimal performance compared with other attacks at low poisoning ratios. WPDA at low poisoning ratios is even more stable than WPDA at high poisoning ratios, such as against CLP, I-BAU and NC. As for VGG19-BN, results illustrate that attacks at high poisoning ratios increase the risk of success against defenses, \textit{i.e.}, a significant decay of ASR at high poisoning ratios. Fig.~\ref{cifar100_tiny_clp_nc}(Left) shows the t-SNE on the mixed testing samples of CIFAR-100 after CLP. The poisoned testing samples are clearly separated from benign testing samples in the target class after CLP, which means the model effectively captures the channels related to the backdoor, causing the attack to fail. However, lots of benign samples in other classes overlap in the feature space, which results in a significant drop of the model's accuracy on benign testing samples.
 
\paragraph{\textbf{Evaluations on Tiny ImageNet}}
Fig.~\ref{tiny_vgg_defense} illustrates the excellent performance of WPDA on Tiny ImageNet after 5 different defense methods. At less than 0.1\% poisoning ratios, most attack methods fail to achcieve successful attacks. While WPDA not only achieves a model accuracy on backdoor samples that surpasses the accuracy on benign samples but also maintains stability after defense. The stability of some attack methods after defense tends to decrease with an increasing poisoning ratio. For instance, the decline in ASR for Input-aware after I-BAU  is greater at a poisoning ratio of 0.05\% compared to a poisoning ratio of 0.1\%.

% after undergoing I-BAU at a poisoning ratio of 0.05\%,   
% Fig.~\ref{all-defense-vgg} illustrates WPDA trained by Tiny ImageNet is very stable, not only achieving successful attacks, but remaining effective after the defenses, even at low poisoning ratios. The results also show that the backdoor attacks at low poisoning ratios increase the stealth of the attack, for example, WPDA's ASR decay at low poisoning ratios is less than that at high poisoning ratios against I-BAU on both PreAct-ResNet18 and VGG19-BN. Not only WPDA, Input-aware trained on PreAct-ResNet18 and VGG19-BN also shows the same performance against NC.
% What needs to be analysed in particular is the performance of WPDA at 0.01\% poisoning ratio after AC. Fig.~\ref{cifar100_tiny_clp_nc}(Right) illustrates that the poisoned testing samples are effectively separated from the samples in the target class. Although the backdoor effect is effectively mitigated by pruning neurons that are highly correlated with the backdoor, the accuracy of the benign testing samples drops substantially. As for NAD, when the model's attention is shifted, few poisoned training samples cannot promote the model to learn the trigger information effectively, leading to a drop in ASR. Although the effectiveness of WPDA is influenced, the accuracy of the model on benign testing samples decays a lot after NC.\\
\paragraph{\textbf{In summary}} Due to inherent variations among datasets, the performance of a single defense method can differ across a single attack method with different datasets. However, as the results indicate, most defense methods struggle to effectively defend backdoor attack methods at low poisoning ratios, underscoring the necessity of developing defense methods specifically designed for low poisoning ratios. Compared to 7 SOTA attack methods, WPDA demonstrates more stable, stealthy and effective performance, especially at low poisoning ratios.

% Most defense methods are difficult to defend against backdoor attacks with low poisoning ratios, which indicates that it is necessary to explore backdoor attacks at low poisoning ratios. Compared to 7 SOTA attack method, WPDA shows more stable and stealthy performance, especially at low poisoning ratios.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
\centering
% \includegraphics[width=3.6in]
\includegraphics[width=3.2in]{figures/tsne-pre-00004--.pdf}
% \includegraphics[width=3.2in]{figures/tsne-pre-01-.pdf}
\caption{t-SNE\cite{van2008visualizing} about 7 SOTA attack methods and WPDA at 0.004\% poisoning ratio.}
\label{tsne-00004-all-attack}
\end{figure}
\section{Analyses}
\label{tsne-kde}
\subsection{Visualization on t-SNE}
Fig.~\ref{tsne-00004-all-attack} illustrates the t-SNE of 7 SOTA attacks and WPDA on PreAct-ResNet18 trained by CIFAR-10 at 0.004\% poisoning ratio. The red circles indicate benign training samples of the target class, the black circles indicate poisoned training samples and the blue circles indicate poisoned testing samples, both of which are labeled as the target class. For BadNets, Blended, Input-aware, SIG, SSBA, LF and WABA, it is evident that the poisoned training samples are close to the benign samples in the target class, while the poisoned testing samples are evenly distributed across the classes. Based on this observation, we can infer that 
the models based on these attack methods only memorize the poisoned training samples rather than learning the features of the trigger, which results in the backdoor not being activated when the poisoned testing samples are used as inputs. 
Regarding WPDA, the poisoned training samples, the benign testing samples in the target class and the poisoned testing samples are relatively clustered in the feature space, indicating that the features extracted by the model from those samples exhibit significant similarity and the model effectively learns the features of the trigger. In summary, WPDA precisely injects trigger information into the key frequency regions, prompting the model to effectively learn the trigger information even at low poisoning ratios. 

\subsection{{Visualization on \texorpdfstring{$l_2$}--distance KDE}}
Kernel Density Estimation (KDE) is a non-parametric statistical method for estimating the Probability Density Function (PDF) that can be used to describe the distribution of data~\cite{gramacki2018nonparametric}. Specifically, KDE is a measure of estimated probability density defined by a kernel function near each data point in the dataset. In KDE, we usually choose a kernel function and a bandwidth parameter to define the similarity between each data point in the dataset and other data points, usually using the Gaussian kernel function, \etc~\\
\hspace*{0.15cm}
To further verify the effectiveness of the WPDA attack, we conduct $l_2$-distance KDE visualization analyses on PreAct-ResNet18 trained by CIFAR-10 at different poisoning ratios. We extract the features of poisoned samples from the `linear' layer in PreAct-ResNet18 and calculate the $l_2$-distance between each poisoned training sample and each poisoned testing sample, then we can obtain multiple lists of $l_2$-distance between each poisoned training sample and all poisoned testing samples, where the number of lists is equal to the number of poisoned training samples and the length of each list is equal to the number of poisoned testing samples. 
Then average the multiple lists of $l_2$-distance and conduct KDE visualization. 
Fig.~\ref{kde} illustrates $l_2$-distance KDE on PreAct-ResNet18 trained by CIFAR-10. The horizontal axis represents the average $l_2$-distance between the poisoned training samples and the poisoned testing samples, and the vertical axis represents the density of each $l_2$-distance value. The $l_2$-distance with a large value means that the features extracted by the model from the poisoned training samples have a large variability from the features extracted from the poisoned testing samples. It is much difficult for the model to predict the poisoned testing samples as target class.
At 0.004\% poisoning ratio, the $l_2$-distance in WPDA are mainly concentrated in small values, which indicates that the features extracted by the model from the poisoned testing samples are similar to those extracted in the poisoned training samples. While, for other attacks, the features extracted by the model from the poisoned testing samples differ from those extracted from the poisoned training samples. As the poisoning ratios increases, leading to a rise in the ASR, $l_2$-distance value in each attack decreases and concentrates gradually, indicating that the modelis progressively learning the trigger information.
\begin{figure}[!ht]
\centering  %图片全局居中
% \captionsetup[subfigure]{labelformat=empty} 
    {
    \includegraphics[width=1.70in]{figures/kde_all_attack_00004_1.pdf}}
    \label{kde-00004}
% \captionsetup[subfigure]{labelformat=empty} 
\hspace{-0.3cm}
    {
    \includegraphics[width=1.70in]{figures/kde_all_attack_01_1.pdf}}
    \label{kde-01}
\caption{$l_2$-distance KDE on CIFAR-10 at 0.004\% poisoning ratio (left) and 1\% poisoning ratio (right).}
\label{kde}
% \vspace{-0.5cm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

Fig.~\ref{The generalization of the model on the trigger information} has demonstrated that models exhibit generalization ability. To confirm our conclusions, we conduct $l_2$-distance KDE visualization on PreAct-ResNet18 by modifying original information intensities $\alpha$ and trigger information intensities $k'$ of the poisoned testing samples.
Fig.~\ref{kde-alpha} shows the $l_2$-distance KDE visualization under different original information intensities $\alpha$. With the increase of the intensity of original information $\alpha$, the $l_2$-distance in feature space between the poisoned testing samples and the poisoned training samples gradually increases. As a result, the original information has a negative effect on the backdoor model, but we can rely on the model's generalization ability to activate the backdoor when the prominence of the trigger is stronger than that of the original information.
Fig.~\ref{kde-k'} shows the $l_2$-distance KDE visualization under different trigger information intensities $k'$. The increase of the trigger information intensity $k'$ can promote the backdoor model to capture the trigger information, which is positive for the activation of the backdoor.

\begin{figure}[!ht]
\centering  %图片全局居中
    \subfigure[$l_2$-distance KDE under different original information intensities $\alpha$]{
    \label{kde-alpha}
    \includegraphics[width=1.6in]{figures/tsne_WPDA_alpha_00004_.pdf}}
    \subfigure[$l_2$-distance KDE under different trigger information intensities $k'$]{
    \label{kde-k'}
    \includegraphics[width=1.6in]{figures/tsne_WPDA_k1_00004_.pdf}}
\caption{$l_2$-distance KDE on CIFAR-10 at 0.004\% poisoning ratio.}
\label{kde-generation}
\end{figure}



% Section~\ref{stealthiness of trigger information} has demonstrated that the model is generalizable. 
% Fig.~\ref{memorizing_pre} shows the the feature distribution under different original information intensities. Both on PreAct-ResNet18 and VGG19-BN, with the increase of the intensity of original information, the difference in feature distribution between the testing samples and the training samples becomes more obvious. As a result, the original information has a negative effect on the backdoor model to activate the backdoor, and WPDA is to promote the model to learn trigger information rather than memorizing backdoor samples. 
% % Therefore, we conclude that the model effectively learns the trigger, rather than memorizing the poisoned samples.
% Fig.~\ref{KDE-PreAct-ResNet18-others} shows the KDE distribution of 7 SOTA methods and WPDA on PreAct-ResNet18 trained by CIFAR-10 at 0.004\% poisoning ratio. As for BadNets, Blended, Input-aware, SIG, SSBA, LF and WABA, the distribution of the average features of the poisoned training samples is quite different from that of the poisoned testing samples. In other words, the model based on these attack methods only remembers the poisoned training samples rather than learn the characteristics of the trigger, which causes the backdoor to not be activated. 
% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=6in]{figures/memorizing_alpha1.png}
% \caption{The KDE visualization based on our method of CIFAR-10 with 0.004\% poisoning ratio. We modify the intensity of original image information to  (First row: Model PreAct-ResNet18; Second row: Model VGG19-BN).}
% \label{memorizing_pre}
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=5in]{figures/tsne00004_1.png}
% \caption{The KDE visualization of different attack methods based on CIFAR-10 with 0.004\% poisoning ratio trained by PreAct-ResNet18.}
% \label{KDE-PreAct-ResNet18-others}
% \end{figure*}

                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     

==> tip/6_conclusion.tex <==
\section{Conclusion}
\label{conclusion}
In this work, a novel frequency-based backdoor attack, WPDA, is proposed. By analyzing the frequency information distribution of datasets based on Wavelet Packet Decomposition (WPD), we infer the key frequency regions which the models would focus on and inject trigger. To promote the model to learn the trigger effectively, we conduct qualitative analyses experiments to design backdoor pattern. Our method not only maintain the naturalness of backdoor samples, but also successfully achieve backdoor attack at extremely low poisoning ratios. 
Besides, we conduct t-SNE to analyze the distribution of the poisoned training samples and the poisoned testing samples in the feature space to vertify the effectiveness of our method. We also conduct $l_2$-distance KDE visualization experiments to observe the $l_2$-distance value of attack methods at different poisoning ratios, demonstrating that WPDA prompts the model to efficiently learn the trigger information rather than memorizing the poisoned training samples at low poisoning ratios.

\section*{Acknowledgments}
The authors would like to thank National Natural Science Foundation of China under grant No.62076213, Shenzhen Science and Technology Program under grants No.RCYX20210609103057050, which support Baoyuan Wu.
